Distributed Synchronous Visualization Design: Challenges and Strategies

We reflect on our experiences as designers of COVID-19 data visualizations working in a distributed synchronous design space during the pandemic. This is especially relevant as the pandemic posed new challenges to distributed collaboration amidst civic lockdown measures and an increased dependency on spatially distributed teamwork across almost all sectors. Working from home being 'the new normal', we explored potential solutions for collaborating and prototyping remotely from our own homes using the existing tools at our disposal. Since members of our cross-disciplinary team had different technical skills, we used a range of synchronous remote design tools and methods. We aimed to preserve the richness of co-located collaboration such as face-to-face physical presence, body gestures, facial expressions, and the making and sharing of physical artifacts. While meeting over Zoom, we sketched on paper and used digital collaboration tools, such as Miro and Google Docs. Using an auto-ethnographic approach, we articulate our challenges and strategies throughout the process, providing useful insights about synchronous distributed collaboration.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> [BELIV 2020] Remote COVID-19 Design/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> [BELIV 2020] Remote COVID-19 Design/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> [BELIV 2020] Remote COVID-19 Design/sections/00-title.tex <==
% \title{Visualizing COVID-19: Remote Ideation}
% \title{Possibilities, Challenges, and Opportunites from a Remote Visualization Design Case}
%\title{Distributed Visualization Design:  Possibilities, Challenges, and Opportunities from Assembling and Collaborating as a Design Team}
\title{Distributed Synchronous Visualization Design:\\Challenges and Strategies}

==> [BELIV 2020] Remote COVID-19 Design/sections/01-authors.tex <==
%% This is how authors are specified in the conference style

%% Author and Affiliation (single author).
%%\author{Roy G. Biv\thanks{e-mail: roy.g.biv@aol.com}}
%%\affiliation{\scriptsize Allied Widgets Research}

%% Author and Affiliation (multiple authors with single affiliations).
%%\author{Roy G. Biv\thanks{e-mail: roy.g.biv@aol.com} %
%%\and Ed Grimley\thanks{e-mail:ed.grimley@aol.com} %
%%\and Martha Stewart\thanks{e-mail:martha.stewart@marthastewart.com}}
%%\affiliation{\scriptsize Martha Stewart Enterprises \\ Microsoft Research}

%% Author and Affiliation (multiple authors with multiple affiliations)
\author{Tatiana Losev\thanks{e-mail: tatiana\_losev@sfu.ca}\\ %
        \scriptsize Simon Fraser University%
\and Sarah Storteboom\thanks{e-mail: sstorteboom@gmail.com}\\ %
     \scriptsize University of Calgary%
\and Sheelagh Carpendale\thanks{e-mail: sheelagh@sfu.ca}\\ %
        \scriptsize Simon Fraser University%
\and Søren Knudsen\thanks{e-mail: sknudsen@ucalgary.ca}\\ %
     \parbox{1.4in}{\scriptsize \centering University of Calgary}}

==> [BELIV 2020] Remote COVID-19 Design/sections/02-abstract.tex <==
%% Abstract section.
\abstract{We reflect on our experiences as designers of COVID-19 data visualizations working in a distributed synchronous design space during the pandemic. This is especially relevant as the pandemic posed new challenges to distributed collaboration amidst civic lockdown measures and an increased dependency on spatially distributed teamwork across almost all sectors. Working from home being ‘the new normal’, we explored potential solutions for collaborating and prototyping remotely from our own homes using the existing tools at our disposal. Since members of our cross-disciplinary team had different technical skills, we used a range of synchronous remote design tools and methods. We aimed to preserve the richness of co-located collaboration such as face-to-face physical presence, body gestures, facial expressions, and the making and sharing of physical artifacts. While meeting over Zoom, we sketched on paper and used digital collaboration tools, such as Miro and Google Docs. Using an auto-ethnographic approach, we articulate our challenges and strategies throughout the process, providing useful insights about synchronous distributed collaboration. 
} % end of abstract

==> [BELIV 2020] Remote COVID-19 Design/sections/10-introduction.tex <==
%% The ``\maketitle'' command must be the first command after the
%% ``\begin{document}'' command. It prepares and prints the title block.

%% the only exception to this rule is the \firstsection command
\firstsection{Introduction}

\maketitle
In this paper, we describe and discuss our experiences of forming and working in a distributed visualization design team. While prior work has discussed visualization design processes~\cite{sedlmair2012design}, it tended to focus on how the visualization community works during face-to-face (co-located) design activities and processes for including users or domain experts. Less attention has been paid to how team collaboration works within teams of visualization designers, be they distributed or co-located.
% Would be great to cite here, but not sure we can find a clear example - thus, the phrasing "our reading".
%Building on the existing body of literature on collaboration in Human-Computer Interaction (HCI) and Computer Supported Collaborative Work (CSCW), w
We discuss our experiences of the differences between co-located and distributed visualization design work specific to our unique needs and experiences in light of an increased reliance on spatially distributed teamwork across almost all sectors. 

Our work was set in motion as part of a provincial response to the COVID-19 pandemic. We were a small team within a broader group of public health researchers who were providing data to government decision-makers during the pandemic. We formed our design team of six members (see Figure \ref{fig:teaser}, members A-F) to support the local health authorities' pandemic response in collaboration with our colleagues at the Centre for Health Informatics at the University of Calgary. As we were a newly acquainted multi-disciplinary team, we found it more beneficial to learn and to discuss the data together in a synchronous environment in the beginning of the project.  
We worked on the design of visualizations of provincial and national COVID-19 data for a public-facing website showing data visualizations of case and policy data. The intention with this site was to inform city- and province-level leaders to assist them in making sense of the status of the public health crisis and the associated data. 
While our team had visualization design expertise, our colleagues provided a wider set of skills and knowledge in fields such as public health, epidemiology, and data science. 
Due to the pandemic, we were unable to meet face-to-face. Instead and against our common work practice, all design team members worked from their home. This situation intensified challenges of distributed collaboration caused by distracting at-home work spaces and a sense of urgency amidst civic lockdown measures.  

Through an auto-ethnographic approach ~\cite{neustaedter2012autobiographical, bullough2001guidelines, duncan2004autoethnography, meyer2018reflection, meyer2020criteria}, we reflect on our experiences of distributed, primarily synchronous ideation and prototyping as a way to identify some challenges in our process of remote visualization design. %Auto-ethnographic research methodology is befitting because its primary evidence base is the unique lived experiences of the researcher(s) \cite{chang2013individual}. This framework was a useful way to discover relevant findings as they emerged via a process of iterative reflection upon our own data that we created throughout synchronous collaborative activities~---~assembling the team, frequent online meetings, data discovery and consultation with health experts, sketching, sharing and brainstorming ideas. The data that we used for our self-study are texts and artifacts from our design activities in Slack conversations, Google Docs, meeting notes, Miro board posts and sketches. 
Our main contribution is an articulation of challenges and strategies for dealing with these while doing distributed visualization design centered on the potential for doing activities, using technologies, and processes for communicating early and often, in order to reduce friction in visualization design teams.
% phase of remote collaboration in visualization design to enable a more fluid geographically distributed workflow.
 
% Due to strict isolation protocols mandated during the crisis, 
We relied on remote design tools and methods to actively design in real-time, often for two hours per day. We aimed to preserve the richness and diversity of co-located collaboration; specifically, the facilitation of face-to-face presence with the ability to view responsive body gestures, facial expressions, and the making and sharing of physical and digital artifacts. 


% %% \section{Introduction} %for journal use above \firstsection{..} instead

% % \cite{hi}

% %  What is this paper?
% In this paper, we describe and discuss our experiences of forming and working in a distributed visualization design team. While prior work has discussed visualization design processes, our reading of the literature suggests our visualization community has tended to focus on face-to-face (co-located) design activities and processes for including users or domain experts. Less attention has been paid to the inside of team co-located collaboration between visualization designers.
% % Would be great to cite here, but not sure we can find a clear example - thus, the phrasing "our reading".
% Building on the existing body of literature on collaboration in Human-Computer Interaction (HCI) and Computer Supported Collaborative Work (CSCW), we discuss the difference between co-located and distributed visualization design work, and describe the challenges and opportunities we experienced.

% Our work was set in motion as part of a provincial response to the COVID-19 pandemic. 
% We formed our design team to support the local health authorities' pandemic response in collaboration with our colleagues at the Centre for Health Informatics at University of Calgary. While our small team had visualization design expertise, our colleagues provided a wider set of skills and knowledge in fields such as public health, epidemiology, and data science. 
% We designed visualizations of provincial and national data as a smaller team among a broader group of public health researchers who were providing data to government decision-makers during the pandemic. The team implemented a public-facing website showing data visualizations of case and policy data to inform city- and province-level sense-making about the status of the public health crisis. 

% As local authorities instituted a public health emergency, we were unable to meet for any face-to-face work and all members were working from their homes.
% The pandemic posed new challenges to distributed collaboration with immense pressure and a sense of urgency amidst civic lockdown measures and an increased reliance on spatially distributed teamwork across sectors. As a response to these unique challenges, we reflect on our experience with distributed, primarily synchronous, visualization design work. 
% % Due to strict isolation protocols mandated during the crisis, 
% We relied on remote design tools and methods to actively design in real-time, often for two hours per day. We aimed to preserve the richness and diversity of co-located collaboration; specifically, the facilitation of face-to-face presence with the ability to view responsive body gestures, facial expressions, and the making and sharing of physical and digital artifacts. 

% Based on autobiographical research approaches~\cite{bullough2001guidelines,duncan2004autoethnography,meyer2018reflection,meyer2020criteria}, we recount our experiences of ideation and prototyping as a way to identify some of the gaps in the process of remote visualization design. This self-study approach is a useful way to discover themes that emerge with reflection upon our distributed collaborative activities~---~assembling the team, frequent online meetings, data discovery and consultation with health experts, sketching, and using synchronous online tools to share and to brainstorm ideas. The reflective practice is based on the documentation of our design activities in Slack conversations, Google Docs, meeting notes, Miro board posts, and our design brief. 

% Our main contribution is an articulation of some of our insights about the
% challenges and opportunities that we experienced while doing distributed  visualization design centered on the potential for doing activities, using technologies, and processes for communicating early and often, in order to reduce friction in visualization design teams.

% % phase of remote collaboration in visualization design to enable a more fluid geographically distributed workflow.




==> [BELIV 2020] Remote COVID-19 Design/sections/20-related-work.tex <==
% Now we have explained what we are doing, our approach/how we are doing it, 
% why that seems important, and also very lightly what has been done in this
% space previously.

% Making explicit that other papers in VIS have used reflection method

%%%%OLD VERSION IS COMMENTED OUT BELOW

\section{Related Work}


This work relates to literature on how to design visualizations; on how to support collaboration through visualizations; and on how to support design in technology-mitigated collaboration. 

\subsection{Designing Visualizations}
Making use of design methodology is widely recognized as important for creating useful and usable visualizations~\cite{munzner2014visualization, sedlmair2012design}.
This echoes the broader discussions about design~\cite{sedlmair2012design}, which span a wide array of concerns and advice about concrete design activities. Some examples that focus on co-located activities include the use of sketching~\cite{ buxton2007sketching, greenberg2011sketching, sturdee2019sketching, roberts2016sketching}; %brainstorming~\cite{};
prototyping with a range of media~\cite{snyder2003paper}, and the use of cards to support ideation~\cite{ideo}. 
A considerable amount of this design work is collaborative in nature ranging from the sharing of work in progress in design critiques~\cite{wolf2006dispelling}, through how people design together such as with co-creating artifacts~\cite{bannon2012design}, to ideas about how to involve people that are affected by a design, for example, through human-centered design~\cite{norman1986user} and participatory design~\cite{bannon2012design}. In addition, there are discussions about how to communicate designs, for example, in creating hand-off documents~\cite{maudet2017design} --- many of which people colloquially refer to as design (studio) praxis. 
In visualization, people have considered how to design for the intended audience such as specific experts or the general public (for example, design study methodology~\cite{sedlmair2012design, mccurdy2016action, meyer2020criteria}), and how to design with these people (for example, user-centered visualization design~\cite{koh2011developing, goodwin2013creative}). Also there are suggestions of potentially useful concrete design activities (for example: those based on constructive visualization~\cite{huron2016using}, those conducted as speculative design workshops~\cite{bressa2019sketching, knudsen2012exploratory}, and the use of pencil-and-paper based sketching of data visualizations~\cite{walny2015exploratory}). There is also advice on how to structure design processes, for example, how to teach visualization design to computer science students using five design sheet method~\cite{roberts2016sketching}), and how to more clearly communicate visualization designs (for example, in designers communicating visualization designs to developers as part of a hand-off process~\cite{walny2020data}). 
These are all extremely informative when at least some of the activities can happen co-located, however, they are less applicable for synchronous distributed design activities. In synchronous distributed design activities, they serve more as goals than as methods.  
These ideas will need to be re-interpreted in the context of synchronous distributed design work.




\subsection{Collaboration and Visualization}

There is a rich body of literature on collaboration in related fields such as human-computer interaction (HCI) and computer supported cooperative work (CSCW). The CSCW matrix (see Table~\ref{tab:cscw-matrix-in-vis-design}), which separates collaborative work along space time axes  is useful for understanding this area~\cite{grudin1994computersupported}. 
%We briefly discuss how this matrix relates to the visualization literature.
Two main areas of the CSCW matrix have been purposefully considered in visualization: co-located synchronous collaboration (Table~\ref{tab:cscw-matrix-in-vis-design}, top-left quadrant) and distributed asynchronous collaboration (Table \ref{tab:cscw-matrix-in-vis-design}, bottom-right quadrant). Although these two modes of collaboration have primarily been studied in isolation --- perhaps due to their different technological basis --- they share many challenges (see for example Isenberg et al.~\cite{isenberg2011collaborative}).
Research exploring co-located collaborative visualization includes  the use of tabletops for collaborative information access, for example, Scott et al.~\cite{scott2003system, scott2004territoriality}, the consideration of tabletop displays for collaborative browsing of hierarchical layouts of photographs~\cite{vernier2002visualization}, for analysis of scientific data~\cite{tobiasz2009lark}, and for exploration of book collections~\cite{thudt2012bohemian}.
More recently, people have considered large, high-resolution displays for supporting collaborative visual analytics (for example, Langner et al.~\cite{langner2019multiple} and Knudsen \& Hornbæk~\cite{knudsen2019pade}). 

Research on visualization for communicating across both space and time (asynchronous distributed) have led to ideas about democratizing visualization by making it accessible to all and to the increasing inclusion of visualizations as a way to communicate data in news media. Sense.us~\cite{heer2007voyagers} and ManyEyes~\cite{viegas2007manyeyes} introduced the collaborative possibilities for visualizations on the web. This type of research situates visualizations in a broader social and societal context. Based on these kinds of systems, Heer \& Agrawala~\cite{heer2008design} provide design considerations for collaborative visualization on the web more broadly. Later, work has shown that structuring the processes in collaborative asynchronous visual analysis can lead to increased analysis quality~~\cite{willett2011commentspace, willett2012strategies}, which might provide ideas for subsequent visualization designs~\cite{hullman2015content}.

While collaborative visualization-based analysis is distinct from collaborative visualization design, the CSCW matrix helps conceptualizing the space of synchronous distributed collaboration in relation to other collaborative contexts. There are also relevant similarities between collaborative visualization-based analysis and visualization design. For example, being able to point to a visualization or part of one is both important when designing and using visualizations~\cite{heer2008creation}. Supporting collaborative use of visualization is an important research direction. However, supporting visualization design in synchronous distributed settings has not yet been discussed. 

% Here, we put all the 'real' table contents. Then the table code below uses it in the right places.
% \newcommand{\sameplacesametime}[0]{\parbox[c]{2.75cm}{same place same time}}}
% \newcommand{\sameplacedifftime}[0]{\parbox[c]{2.75cm}{same place different time}}}
% \newcommand{\diffplacesametime}[0]{\parbox[c]{2.75cm}{different place same time}}}
% \newcommand{\diffplacedifftime}[0]{\parbox[c]{2.75cm}{different place different time}}}

\begin{table}[tb]
\centering
\caption{CSCW matrix for consideration in visualization design.}
% \begin{tabular}{@{}c|p{3cm}p{3cm}@{}}
\begin{tabular}{@{}p{1.85cm}|p{2.75cm}p{2.75cm}@{}}
\toprule 
& \parbox[c]{2.75cm}{Same time\\(synchronous)} & \parbox[c]{2.75cm}{Different time\\(asynchronous)} \\ \midrule

% \parbox[c]{2.0cm}{Same place\\(co-located)}
\raggedright Same place (co-located)
& same place same time & same place different time \\[0.5cm]
% \parbox[c]{2.0cm}{Different place\\(distributed)}
Different place (distributed)
& different place same time & different place different time \\ 
\bottomrule
\end{tabular}
\label{tab:cscw-matrix-in-vis-design}
\end{table}

\subsection{Collaborative Design of Visualizations}
While the visualization literature includes many discussions about design~\cite{beecham2020design,bigelow2014reflections,goodwin2013creative,koh2011developing,mccurdy2016action,mckenna2014design,mckenna2017worksheets,meyer2020criteria,munzner2014visualization,sedlmair2012design,walny2020data,hall2020design}, the focus is on the design processes rather than the collaborative process. The collaborations discussed  tend to focus on how visualization researchers collaborate in long-term projects with domain experts. For example, while the term ``collaboration'' (and related forms) is used 34 times in the design studies paper~\cite{sedlmair2012design}, it is only used a single time in the section that discusses the ``core phase'' of the design study methodology. Discussions about collaborative design thinking seem to be missing. 

Similarly, in CSCW literature, while there are discussions about many different types of work, the focus has been on distributed asynchronous and co-located synchronous. We are interested in distributed synchronous design activities.   

\subsection{Collaborative Design Processes}
\revision{There is CSCW literature about collaborative design processes (for some examples see~\cite{tausch2015thinking, fischer2004social, hilliges2007designing, yu2011cooks, arias2000transcending, bratteteig2012spaces, obendorf2009inter}). However, the focus is still about collaborative design when co-location is part of the design process. 
For example, some have explored technology mitigated collaborations through tabletop display tools~\cite{hilliges2007designing, bratteteig2012spaces}, and through investigating the impact of technology based feedback about the group creative design process~\cite{tausch2015thinking}. One suggestion is to explore the use of the crowd in design processes\cite{yu2011cooks}.
Visualization has been used to provide feedback on speaking times and speaking turns during collaboration~\cite{ bergstrom2007conversation}.}

\revision{There is some exploration of the space we are interested in – the space of how to re-kindle the benefits of co-located collaboration in a technology-supported, synchronous distributed situation. Arias et al.~\cite{arias2000transcending} start by acknowledging the complex design problems often require group solutions and articulates needed design support for urban design problems. Both Fischer~\cite{fischer2004social} and Obendorf et al.~\cite{obendorf2009inter} consider the complexity of team-based design needs where teams must cope with difference in time, space, and knowledge and make a call for deeper exploration of the needs of these types of design teams. Our work, which describes our experiences of the challenges of collaborative synchronous, distributed technology-mediated design, and a range of strategies for dealing with these challenges, contributes to this larger call for research.}  




% Considerations for design methodology are widely recognized as important for creating useful and usable
% % i do not know about this sensible?, and sensible 
% visualization products~\cite{munzner2014visualization}.
% % Should we add more citations above?
% This echoes broader discussions of design, which span a wide array of %concerns such as 
% concrete design activities % this footnote dates the paper only relevent for this summer \footnote{This is also the topic of a IEEE VIS 2020 workshop: \url{https://visactivities.github.io/\#topics-and-submissions}}
% such as sketching~\cite{greenberg2011sketching,sturdee2019sketching,roberts2016sketching}, brainstorming,  prototyping with a range of media~\cite{snyder2003paper}, and design phases~\cite{buxton2007sketching}.  
% % studio practice  how designers organise their work spaces~\cite{},
% % I have realised what people talk about as design studio practice is more of an umbrella term so it does not make sense to add that to the list. 
% Also a considerable amount of design work is collaborative in nature, ranging from 
% the sharing of work in progress in design critiques~\cite{wolf2006dispelling}, and how people design together such as through co-creating artifacts~\cite{bannon2012design},
% to ideas about how to involve people that are affected by a design, for example, through human-centered design~\cite{norman1986user} and participatory design~\cite{bannon2012design}. In addition, there are discussions about how to communicate designs, for example, in creating hand-off documents~\cite{maudet2017design} --- many of which people colloquially refer to as design (studio) praxis.
% \newpage
% In visualization, people have considered how to design for end-users (for example, design study methodology~\cite{sedlmair2012design,mccurdy2016action,meyer2020criteria}), how to design with end-users (for example, user-centered visualization design~\cite{koh2011developing,goodwin2013creative}), potential concrete design activities (for example, based on constructive visualization~\cite{huron2016using}, conducting speculative design workshops~\cite{bressa2019sketching,knudsen2012exploratory}, and pen-and-paper based sketching of data visualizations~\cite{walny2015exploratory}), how to structure design processes (for example, teaching visualization design to computer science students using five design sheet method~\cite{roberts2016sketching}), and how to clearly communicate visualization designs (for example, in designers communicating visualization designs to developers as part of a hand-off process~\cite{walny2020data}).
% We discuss related literature under
% % these 2 lists read as different things - 2nd list relates to the rest of this section soooo ... First, concrete activities that one can do in visualization design. Second, how designers collaborate and where they do it. Third, how people besides the designers themselves are part of the process. 
% % (users, stakeholders, programmers (for example, as in Walny et al.~\cite{walny2020data})).
% Collaboration and Visualization, and Collaborative Visualization Design.
% %, and distributed design work.
% %more broadly.

% \subsection{Collaboration and Visualization}
% There is a rich body of literature on collaboration in visualization in related fields such as HCI and CSCW. The CSCW matrix (see Table~\ref{tab:cscw-matrix-in-vis-design}) has been useful for understanding this area~\cite{grudin1994computersupported}. 
% %We briefly discuss how this matrix relates to the visualization literature.
% Two main areas of the CSCW matrix have been purposefully considered in visualization: co-located synchronous collaboration (Table \ref{tab:cscw-matrix-in-vis-design}, top-left quadrant) and distributed asynchronous collaboration (Table \ref{tab:cscw-matrix-in-vis-design}, bottom-right quadrant). Although these two modes of collaboration have primarily been studied in isolation --- perhaps due to their different technological basis --- they share many challenges (see for example Isenberg et al.~\cite{isenberg2011collaborative}).

% %%% I still think we could remove this whole paragraph 
% Several HCI researchers considered collaborative visualization in terms of horizontal displays, notable publications include:
% %%--- for example, the \textit{ACM International Conference on Interactive Tabletops and Surfaces (ITS)} conference was formed in 2006. At that time, 
% studies on the use of tabletops for collaborative information access, for example, Scott et al.~\cite{scott2003system,scott2004territoriality}, the consideration of tabletop displays for collaborative browsing of hierarchical layouts of photographs~\cite{vernier2002visualization}, for analysis of scientific data~\cite{tobiasz2009lark}, and for exploration of book collections~\cite{thudt2012bohemian}.
% More recently, people have considered large, high-resolution displays for supporting collaborative visual analytics (for example, Langner et al.~\cite{langner2019multiple} and Knudsen \& Hornbæk~\cite{knudsen2019pade}).% \soren{what are the benefits of co-located sync collab?}

% At the same time, visualizations have become common as ways to communicate data in news media. Sense.us~\cite{heer2007voyagers} and ManyEyes~\cite{viegas2007manyeyes} introduced the collaborative possibilities for visualizations on the web. These situate visualizations in a broader social and societal context. Based on  systems like Sense.us, ManyEyes, Heer \& Agrawala~\cite{heer2008design} provide design considerations for collaborative visualization on the web more broadly. We note interesting points between their considerations and other quadrants in the CSCW matrix. For example, we think that people have a need for pointing to visual marks in a visualization across all modes of collaboration. However, visualizations shared online have a much stronger need for directly supporting this~\cite{heer2008creation}.
% Using visualizations to communicate data online clearly has been shown to offer societal benefits. %% But there are also more direct benefits from collaboration.
% Willett et al.~\cite{willett2011commentspace,willett2012strategies} show that structuring the processes in collaborative asynchronous visual analysis can lead to increased analysis quality. Hullman et al.~\cite{hullman2015content} suggest comments on online visualizations can be used in the visualization design process. 

% %% i DO NOT GET THE PURPOSE OF THIS PARAGRAPHB
% % While others before us have discussed the relationship between the collaboration and visualization~\cite{heer2008creation,isenberg2011collaborative}, we ask what might be learned from this body of work for distributed visualization design. We conclude that many researchers have argued that co-located synchronous visualization work has great benefits, and that these arguments are supported by empirical data. Additionally, the number of visualizations shown to a mass online audience is an even stronger indication of value. Thus, in seeking to understand collaborative \textit{use} of visualization, one might consider several collaboration modes for the different value they bring, as suggested previously~\cite{roberts2014visualization}. 

% %% this also is for a different paper that is not what has been written. 
% %Following this understanding, it is relevant to ask how and to which extent it makes sense to compare visualization \textit{use} and visualization \textit{design}. While design is different from use and should be informed from knowledge and observation, we think that an important element of design is \textit{imagined} use --- to extrapolate what the designer knows to the design situation and to clearly articulate this understanding to collaborating designers and other team members. While a part of visualization \textit{use} might be internal to a person reading a visualization~\cite{heer2008design}, we expect that visualization designers will need to be able to understand and articulate aspects of use more clearly. 
% %From this understanding, we next discuss visualization design as a collaborative activity.


% % Lets recreate the normal cscw matrix (https://www.researchgate.net/figure/CSCW-Matrix-Johansen-1988_fig2_287217634) but with examples of visalization design 



% \subsection{Collaborative Visualization Design}
% In our reading of the visualization literature~\cite{beecham2020design,bigelow2014reflections,goodwin2013creative,koh2011developing,mccurdy2016action,mckenna2014design,mckenna2017worksheets,meyer2020criteria,munzner2014visualization,sedlmair2012design,walny2020data,hall2020design}, the visualization community does not tends to focus on the collaborative -- that is between visualization designers --  nature of our design processes. Collaborative visualization design seems to focus on how visualization researchers collaborate in long-term projects with domain experts. For example, while the term ``collaboration'' (and related forms) is used 34 times in the design studies paper~\cite{sedlmair2012design}, only one of those times it is used in the section that discusses the ``core phase'' of the design study. Reading the body of literature on visualization design would suggest that visualization researchers create designs almost in isolation. We do not think this is the case. Rather, we think the collaborative nature of the core phases of the visualization design process is merely not articulated. While we acknowledge that some of these core design processes that can be done fruitfully with external collaborators, they can also be done independently. We seem to lack specific written discussions on how visualization designers themselves might collaborate. 

% % Here, we put all the 'real' table contents. Then the table code below uses it in the right places.
% \newcommand{\sameplacesametime}[0]{same place same time}
% \newcommand{\sameplacedifftime}[0]{same place different time}
% \newcommand{\diffplacesametime}[0]{different place same time}
% \newcommand{\diffplacedifftime}[0]{different place different time}

% \begin{table}[tb]
% \centering
% \begin{tabular}{@{}c|p{2.75cm}p{2.75cm}@{}}
% \toprule
% & \parbox{2.75cm}{\center{Same time\\(synchronous)}} & \parbox{2.75cm}{\center{Different time\\(asynchronous)}} \\ \midrule
% %\rotatebox[origin=c]{0}{\parbox{2.75cm}{\center{Same place\\(co-located)}}}
% \rotatebox[origin=c]{0}{\parbox{2.0cm}{\center{Same place\\(co-located)}}}
% %\rotatebox[origin=c]{90}{\parbox{2.75cm}
% %{\center{Same place\\(co-located)}}
% &\sameplacesametime{} & \sameplacedifftime{} \\
% \rotatebox[origin=c]{0}{\parbox{2.0cm}{\center{Different place\\(distributed)}}}
% %\rotatebox[origin=c]{90}{\parbox{2.75cm}
% %{\center{Different place\\(remote / distributed)}}
% &\diffplacesametime{} & \diffplacedifftime{} \\ \bottomrule
% \end{tabular}
% \caption{CSCW matrix for consideration in visualization design.}
% \label{tab:cscw-matrix-in-vis-design}
% \end{table}


% %%% would like to include these quotes but do not know what paper they come from - so am removing
% \begin{quote}
% ``There are many reasons for using lo-fi sketching. Not only does it help users make explicit their thoughts, but it also helps them to \textit{share} their thoughts with others and \textit{collaboratively} work on a design.''
% \end{quote}
% Later,
% \begin{quote}
% ``Ideas emerge by thinking, talking with other people, reading relevant literature, gaining inspiration from other domains, resting and not rushing, reflecting and \textit{collaborating}.'' \cite{roberts2016sketching}, our emphases.
% \end{quote}


% What we can find about collaborative visualization design relates to specific activities designers might use. For example, in Huron et al.~\cite{huron2016using} the people partaking in a constructive design session might ``\textit{collaboratively} discuss whether or not they have represented these features in their visualization.'' Similarly, Roberts et al.~\cite{roberts2016sketching} do note importance of discussion between designers -- \textit{``There are many reasons for using lo-fi sketching. Not only does it help users make explicit their thoughts, but it also helps them to \textit{share} their thoughts with others and \textit{collaboratively} work on a design.''}.
% We think that there is a place for more experience reports that describe collaborative design practices in visualization. For example, when more than a single person is engaging in a visualization design process: How often do they meet and for how long? What do they do in these meetings and do they structure them in a specific manner? Do they frequently exchange information between meetings? How is the division of design labor?
% In our work, we attempt to shed more light on this from the perspective of distributed visualization design work. We think the need to ``go remote'' has ignited these questions, as we have participated in many design processes previously without seeking out this knowledge. 


% %For this reason, we finish this section by looking to discussions of design work with a focus on distributed processes.


% %%%%% the rest of this for another time, another paper ...
% % \subsection{Distributed design work}
% % The first understanding: collaboration is needed to increase opportunities for creativity. More people can be more creative. The renaisance scholar is no more~\cite{arias2000transcending}

% % We are inspired by discussions of workspace awareness~\cite{gutwin2002descriptive}.

% % We are inspired by discussions of trade-offs between support for individuals and groups~\cite{gutwin1998design}.

% % Design and collaboration
% % \cite{arias2000transcending,bao2018interplay,chiu2002organizational,everitt2003two,frich2018twenty,keinonen2009immediate,koutsabasis2012value,kvan2000collaborative,paulini2013design,schonheyder2018use}

% % Remote vs colocated design
% % \cite{eris2014comparative,gul2009cocreating,gul2009cocreatinga,hong2019architectural}


% % What is it

% % What has been tried

% % What can we take from this to understand how we might do remote visualization design.

% %\subsection{Summary}
% %In starting our distributed design process, we consulted with the literature outlined above. However, this body of literature offers limited advice for how to organize collaborative visualization design processes. Instead, we combined our experience from our own prior design processes in visualization design and beyond, with our readings about visualization design and distributed design. In the following, we describe our experiences with doing distributed visualization design and offer our advice through an articulation of challenges and opportunities.

% %\subsection{Notes}
% % Design team

% % Solutions that worked in other remote design and collaboration contexts
% % - leveraging face-to-face interaction but using the camera
% % - leveraging 'gestures'

% % Similar challenges and solutions that we found in related work

% % Being able to see real-time sketching from other team members

% % Distinguishing different environments: co-located, distributed

% % Team structure and work flow

% % While descriptions and discussions of visualization design has tended to assume co-located design teams, designers clearly need to carry out some work independently and in different locations. Prior work in other fields have shed light on this. However, there is important work to be done in considering these contexts for visualization design processes. We provide a first understanding and conceptualization of this area.

% % We articulate how we collaborated remotely to design interactive visualizations. While no (I think) work on visualization design process articulate whether design processes have been co-located or remote, our reading of the field leaves the impression that most design has happened co-located. In this paper, we discuss purely distributed design processes, and so, look to other fields of design that discuss distributed design. Similarly relevant, we have dabbled in both synchronous and asynchronous design processes .

% % It is worth noting that these different modes of collaboration have been described in the field of computer supported collaborative work (CSCW) as the CSCW matrix. See Figure \ref{tab:cscw-matrix-in-vis-design}.


% % Now we have explained what we are doing, our approach/how we are doing it, 
% % why that seems important, and also very lightly what has been done in this
% % space previously.

% % Making explicit that other papers in VIS have used reflection method

% % \section{Related work}
% % Considerations for design methodology are widely recognized as important for creating useful and usable
% % % i do not know about this sensible?, and sensible 
% % visualization products~\cite{munzner2014visualization}.
% % % Should we add more citations above?
% % This echoes broader discussions of design, which span a wide array of %concerns such as 
% % concrete design activities % this footnote dates the paper only relevent for this summer \footnote{This is also the topic of a IEEE VIS 2020 workshop: \url{https://visactivities.github.io/\#topics-and-submissions}}
% % such as sketching~\cite{greenberg2011sketching,sturdee2019sketching,roberts2016sketching}, brainstorming,  prototyping with a range of media~\cite{snyder2003paper}, and design phases~\cite{buxton2007sketching}.  
% % % studio practice  how designers organise their work spaces~\cite{},
% % % I have realised what people talk about as design studio practice is more of an umbrella term so it does not make sense to add that to the list. 
% % Also a considerable amount of design work is collaborative in nature ranging from 
% % the sharing of work in progress in design critiques~\cite{wolf2006dispelling}), through how people design together such as through co-creating artifacts~\cite{bannon2012design},
% % to ideas about how to involve people that are affected by a design, for example, through human-centered design~\cite{norman1986user} and participatory design~\cite{bannon2012design}). In addition there are discussions about how to communicate designs, for example, in creating hand-off documents~\cite{maudet2017design}) --- many of which people colloquially refer to as design (studio) praxis.

% % In visualization, people have considered how to design for end-users (for example, design study methodology~\cite{sedlmair2012design,mccurdy2016action,meyer2020criteria}), how to design with end-users (for example, user-centered visualization design~\cite{koh2011developing,goodwin2013creative}), potential concrete design activities (for example, based on constructive visualization~\cite{huron2016using}, conducting speculative design workshops~\cite{bressa2019sketching,knudsen2012exploratory}, and pen-and-paper based sketching of data visualizations~\cite{walny2015exploratory}), how to structure design processes (for example, teaching visualization design to computer science students using five design sheet method~\cite{roberts2016sketching}), and how to clearly communicate visualization designs (for example, in designers communicating visualization designs to developers as part of a hand-off process~\cite{walny2020data}).
% % Our work relates to three important aspects of the design literature: 
% % % these 2 lists read as different things - 2nd list relates to the rest of this section soooo ... First, concrete activities that one can do in visualization design. Second, how designers collaborate and where they do it. Third, how people besides the designers themselves are part of the process. 
% % % (users, stakeholders, programmers (for example, as in Walny et al.~\cite{walny2020data})).
% % collaboration and visualization, collaborative visualization design, and distributed design work.
% % %more broadly.

% % \subsection{Collaboration and Visualization}
% % There is a rich body of literature on collaboration in visualization in related fields such as HCI and CSCW. The CSCW matrix (see Table 2) has been useful for understanding this area~\cite{grudin1994computersupported}. 
% % We briefly discuss how this matrix relates to the visualization literature.
% % Two main areas of the CSCW matrix have been purposefully considered in visualization: co-located synchronous collaboration (Table \ref{tab:cscw-matrix-in-vis-design}, top-left quadrant) and distributed asynchronous collaboration (Table \ref{tab:cscw-matrix-in-vis-design}, bottom-right quadrant). Although these two modes of collaboration have primarily been studied in isolation --- perhaps due to their different technological basis --- they share many challenges (see for example Isenberg et al.~\cite{isenberg2011collaborative}).

% % %%% I still think we could remove this whole paragraph 
% % Several HCI researchers started to study horizontal tabletop displays --- for example, the \textit{ACM International Conference on Interactive Tabletops and Surfaces (ITS)} conference was formed in 2006. At that time, studies on the use of tabletop surfaces had already appeared at major publication venues (for example, Scott et al.~\cite{scott2003system,scott2004territoriality}). In visualization, people have, for example, considered tabletop displays for collaborative browsing of hierarchical layout of photographs~\cite{vernier2002visualization}, analysis of scientific data~\cite{tobiasz2009lark}, and exploration of book collections~\cite{thudt2012bohemian}.
% % More recently, people have considered large, high-resolution displays for supporting collaborative visual analytics (for example, Langner et al.~\cite{langner2019multiple} and Knudsen \& Hornbæk~\cite{knudsen2019pade}). \soren{what are the benefits of colocated sync collab?}

% % At the same time, visualizations have become common as ways to communicate data in news media to a mostly lay audience. Sense.us~\cite{heer2007voyagers} and ManyEyes~\cite{viegas2007manyeyes} introduced the collaborative possibilities for visualizations on the web. These situate visualization in a broader social and societal context. Based on Sense.us, ManyEyes, and other systems, Heer \& Agrawala~\cite{heer2008design} provide design considerations for collaborative visualization on the web more broadly. We note interesting points of between their considerations and other quadrants in the CSCW matrix. For example, we think that people have a need for pointing to visual marks in a visualization across all modes of collaboration. However, visualizations shared online have a much stronger need for directly supporting this.
% % % \cite{heer2008creation}
% % Using visualizations to communicate data online clearly poses societal benefits. But there are also more direct benefits from collaboration.
% % Willett et al.~\cite{willett2011commentspace,willett2012strategies} show that structuring the processes in collaborative asynchronous visual analysis can lead to increased analysis quality. Hullman et al.~\cite{hullman2015content} suggests comments on online visualizations can be used in the visualization design process. 

% % While others before us have discussed the relationship between the collaboration and visualization~\cite{heer2008creation,isenberg2011collaborative}, we ask what might be learned from this body of work for distributed visualization design. We conclude that many researchers have argued that colocated synchronous visualization work has great benefits, and that these arguments are supported by empirical data. Additionally, the number of visualizations shown to a mass online audience is an even stronger indication of value. Thus, in seeking to understand collaborative \textit{use} of visualization, one might consider several collaboration modes for the different value they bring, as suggested previously~\cite{roberts2014visualization}. 

% % Following this understanding, it is relevant to ask how and to which extent it makes sense to compare visualization \textit{use} and visualization \textit{design}. While design is different from use and should be informed from knowledge and observation, we think that an important element of design is \textit{imagined} use --- to extrapolate what the designer knows to the design situation and to clearly articulate this understanding to collaborating designers and other team members. While a part of visualization \textit{use} might be internal to a person reading a visualization~\cite{heer2008design}, we expect that visualization designers will need to be able to understand and articulate aspects of use more clearly. 
% % From this understanding, we next discuss visualization design as a collaborative activity.


% % % Lets recreate the normal cscw matrix (https://www.researchgate.net/figure/CSCW-Matrix-Johansen-1988_fig2_287217634) but with examples of visalization design 

% % % Here, we put all the 'real' table contents. Then the table code below uses it in the right places.
% % \newcommand{\sameplacesametime}[0]{same place same time}
% % \newcommand{\sameplacedifftime}[0]{same place different time}
% % \newcommand{\diffplacesametime}[0]{different place same time}
% % \newcommand{\diffplacedifftime}[0]{different place different time}

% % \begin{table}[tb]
% % \centering
% % \begin{tabular}{@{}c|p{2.75cm}p{2.75cm}@{}}
% % \toprule
% % & \parbox{2.75cm}{\center{Same time\\(synchronous)}} & \parbox{2.75cm}{\center{Different time\\(asynchronous)}} \\ \midrule
% % \rotatebox[origin=c]{90}{\parbox{2.75cm}{\center{Same place\\(colocated)}}}
% % &\sameplacesametime{} & \sameplacedifftime{} \\
% % \rotatebox[origin=c]{90}{\parbox{2.75cm}{\center{Different place\\(remote / distributed)}}}
% % &\diffplacesametime{} & \diffplacedifftime{} \\ \bottomrule
% % \end{tabular}
% % \caption{The CSCW matrix applied to our previous visualization design processes.}
% % \label{tab:cscw-matrix-in-vis-design}
% % \end{table}

% % \subsection{Collaborative visualization design}
% % In our reading of the visualization literature~\cite{beecham2020design,bigelow2014reflections,goodwin2013creative,koh2011developing,mccurdy2016action,mckenna2014design,mckenna2017worksheets,meyer2020criteria,munzner2014visualization,sedlmair2012design,walny2020data,hall2020design}, the visualization community tends to gloss over the collaborative nature of our design processes. Collaborative visualization design seems to (only) imply visualization researchers collaborating in long-term projects with domain experts. For example, while the term ``collaboration'' (and related forms) is used 34 times in the seminal design studies paper~\cite{sedlmair2012design}, only one of those times is it used in the section that discusses the ``core phase'' of the design study. Reading the body of literature on visualization design would suggest that visualization researchers create designs almost in isolation. We do not think this is the case. Rather, we think the collaborative nature of the core phases of the visualization design process is un-articulated. While we acknowledge that some of the processes that can be done with external collaborators can also be done independently, we seem to lack specific written advice for how visualization designers themselves might collaborate. 

% % What we can find about collaborative visualization design relates to specific activities designers might use. For example, Huron et al.~\cite{huron2016using} people partaking in a constructive design session might ``\textit{collaboratively} discuss whether or not they have represented these features in their visualization.'' Similarly, Robertson et al.~\cite{roberts2016sketching}:

% % \begin{quote}
% % ``There are many reasons for using lo-fi sketching. Not only does it help users make explicit their thoughts, but it also helps them to \textit{share} their thoughts with others and \textit{collaboratively} work on a design.''
% % \end{quote}
% % Later,
% % \begin{quote}
% % ``Ideas emerge by thinking, talking with other people, reading relevant literature, gaining inspiration from other domains, resting and not rushing, reflecting and \textit{collaborating}.'' (our emphases)
% % \end{quote}

% % We miss advice or experience reports that describe collaborative design practices in visualization. For example, when more than a single person engaging in a visualization design process: How often do they meet and for how long? What do they do in these meetings and do they structure them in a specific manner? Do they frequently exchange information between meetings? How is the division of design labor?

% % In our work, we attempt to shed more light on this from the perspective on distributed visualization design work. We think the need to ``go remote'' have ignited these questions, as we have participated in many design processes previously without seeking out this knowledge. For this reason, we finish this section by looking to discussions of design work with a focus on distributed processes.

% % \subsection{Distributed design work}
% % The first understanding: collaboration is needed to increase opportunities for creativity. More people can be more creative. The renaisance scholar is no more~\cite{arias2000transcending}

% % We are inspired by discussions of workspace awareness~\cite{gutwin2002descriptive}.

% % We are inspired by discussions of trade-offs between support for individuals and groups~\cite{gutwin1998design}.

% % Design and collaboration
% % \cite{arias2000transcending,bao2018interplay,chiu2002organizational,everitt2003two,frich2018twenty,keinonen2009immediate,koutsabasis2012value,kvan2000collaborative,paulini2013design,schonheyder2018use}

% % Remote vs colocated design
% % \cite{eris2014comparative,gul2009cocreating,gul2009cocreatinga,hong2019architectural}


% % What is it

% % What has been tried

% % What can we take from this to understand how we might do remote visualization design.

% % %\subsection{Summary}
% % %In starting our distributed design process, we consulted with the literature outlined above. However, this body of literature offers limited advice for how to organize collaborative visualization design processes. Instead, we combined our experience from our own prior design processes in visualization design and beyond, with our readings about visualization design and distributed design. In the following, we describe our experiences with doing distributed visualization design and offer our advice through an articulation of challenges and opportunities.

% % %\subsection{Notes}
% % % Design team

% % % Solutions that worked in other remote design and collaboration contexts
% % % - leveraging face-to-face interaction but using the camera
% % % - leveraging 'gestures'

% % % Similar challenges and solutions that we found in related work

% % % Being able to see real-time sketching from other team members

% % % Distinguishing different environments: co-located, distributed

% % % Team structure and work flow

% % % While descriptions and discussions of visualization design has tended to assume co-located design teams, designers clearly need to carry out some work independently and in different locations. Prior work in other fields have shed light on this. However, there is important work to be done in considering these contexts for visualization design processes. We provide a first understanding and conceptualization of this area.

% % % We articulate how we collaborated remotely to design interactive visualizations. While no (I think) work on visualization design process articulate whether design processes have been co-located or remote, our reading of the field leaves the impression that most design has happened co-located. In this paper, we discuss purely distributed design processes, and so, look to other fields of design that discuss distributed design. Similarly relevant, we have dabbled in both synchronous and asynchronous design processes .

% % % It is worth noting that these different modes of collaboration have been described in the field of computer supported collaborative work (CSCW) as the CSCW matrix. See Figure \ref{tab:cscw-matrix-in-vis-design}.



==> [BELIV 2020] Remote COVID-19 Design/sections/25-our-challenge.tex <==
\section{Synchronous Distributed Visualization Design}

Amid the COVID-19 lockdown, we were faced with the urgent challenge to design a useful COVID-19 visualization. We were confronted with the reality that our familiar co-located team-based collaboration design approaches could not be directly applied in our enforced distributed but synchronous realm.
While this was a challenge in many ways, we managed to reach an effective design process. Through the use of a reflective auto-ethnographic research approach, we have obtained a deeper understanding of these challenges.
% Before discussing these, w
We first describe our research approach. 

\subsection{Methodology: Reflective Auto-Ethnography}
\revision{We conducted a team-based self-study for this project by combining an auto-ethnographic research approach~\cite{chang2013individual} with hermeneutic phenomenology~\cite{van2016researching}. Auto-ethnographic research is befitting because its evidence base is the direct narrative of the people involved~\cite{chang2013individual}. Hermeneutic phenomenology complements this as it studies the meanings of lived experience through self-reflection, writing, and discussion~\cite{van2016researching,laverty2003hermeneutic}.
Together, these approaches deepened our understanding of our experience as a team of designers creating visualizations together in a synchronous distributed context. Though more commonly seen in the social sciences, we benefit from these qualitative research approaches. They enable us to focus on our unique experiences of designing visualizations in a synchronous distributed setting through the discovery of themes that occurred in our non-linear collaborative practice. }

% Provided that data visualization methods and processes are often not linear and context specific, o

% ur research findings enrich a shared understanding of diverse socio-cultural dimensions. The themes we extracted from our account offer an example to the members of the viz community who may identify with and acknowledge similar experiences that they too had, which serve to amplify an experiential evidence base to inform future visualization research and methodology in this domain.}


\subsection{Demographics: Our Team Members}
\revision{Our group of designers worked together, as a team, for the first time, though some team members (AB, AEF, ABC, BC, and BD --- also shown in Figure \ref{fig:teaser}) had worked together previously on separate projects. The team dynamics and the social setting of the lockdown were novel to the whole team. The domain specific data and the needs of the project had yet to be learned. Thus, the team needed to get acquainted with one another as well as the data. We found that spending more time together in a synchronous setting facilitated an immediate peer-to-peer learning, and improved our communication --– in our experience, this was the most suitable way for us to connect, to build personal relationships in our group, and to improve group synergy. Initially, team members A, E, and F discussed the project for about two weeks, followed by members A and B discussing possible additional members to balance skills in data visualization, design, public health, and programming (see Table 2). Team member A assembled the team and called the first team meeting.}

\subsection{Our Process, Data, and Analysis}
\revision{Following an auto-ethnographic approach, the data is both a result of our process and fueled it; therefore, we discuss them as intertwined. We looked closely into the process of our visualization project by analyzing our own experiential data and project artifacts~\cite{chang2013individual,creswell2016qualitative,laverty2003hermeneutic}. In auto-ethnography we are both the participants and the researchers --- through a self-reflexive process~\cite{chang2013individual,{van2016researching}}, we examine our shared experience as a multi-disciplinary team of designers working towards gaining a deeper understanding of our experience. Doing so, we questioned: \emph{how has distributed collaboration shaped our experience of synchronous design processes?}}

%% need text to go with this
% As a first and important step, we acknowledged our relationships that may contribute to personal biases relevant to the project and detailed our previous experience of designing visualization and how it impacted our contributions to the project

\revision{Our process was as follows: We continuously collected process data and members of the team kept regular day-by-day written team notes; the team's visualization sketches were collectively stored on a Miro board; 
%(for an example see Figure~\ref{sketch.fig}). 
our design brief on Google Docs and the Slack history texts were gathered and reviewed; we created a visual timeline from our Slack history; we formulated questions to guide our inquiry and reflection based on our collected data and previous personal experiences relevant to visualization design and health communications; we characterized, analyzed and reflected on our texts, discussed the texts, and generated new texts;
we held reflective discussions and documented this in our notes in Google Docs; themes that emerged in our text and from our reflective dialogue were grouped; through our reflections, we interpreted our documented themes and continued to write these reflections on our account; we corroborated collective written experiences with one another through further discussion to validate the findings. Lastly, we wrote this paper by detailing our experiences and findings by repeatedly going through the steps above.}



% \begin{itemize} 
% %[noitemsep]
% \item We collected our data – regular day-by-day written team notes, team's visualization sketches, design brief, and Slack history texts. We created a visual timeline from our Slack history
% \item We acknowledged our relationships that contributed to personal biases relevant to the project
% \item We wrote questions to guide our study and reflection based on our collected data and previous personal experiences relevant to visualization work and health
% \item We acknowledged and detailed our previous experience of designing visualization and how it impacted our contributions to the project
% \item We characterized, analyzed and reflected on our texts, discussed the texts, and generated new texts
% \item We held reflective discussions and documented the notes in Google Docs; themes that emerged in our text and from our reflective dialogue were grouped
% \item We interpreted our documented themes and continued to write our account
% \item We corroborated collective written experiences with one another through further discussion to validate the findings
% \item We wrote this paper detailing our experience and findings after cycling through the steps above
% \end{itemize}

\begin{table}[tb]
\centering
\caption{Overview of our team.}
\begin{tabular}{@{}llp{4.5cm}@{}}
\toprule
Team member & Role         & Expertise in use                                               \\ \midrule
A       & PI           & Visualization, design, programming, management, communication       \\
B       & PI           & Visualization, design                                                  \\
C       & Design lead  & Visualization, design                                           \\
D       & Designer     & Public health, design                                         \\
E       & Intern       & Visualization, programming                                    \\
F       & Intern       & Visualization, programming                                    \\ \bottomrule
\end{tabular}
\label{tab2}
% I would like to make a better version of this for camera ready. I imagine you could show a column for each expertise, and then have a vertical label across the column that describes the skill
\label{tab:overview-of-designers}
\end{table}



 \subsection{Our Context}
March 13, 2020, two days before a local state of emergency was announced, the office of the mayor requested help from the Centre for Health Informatics to get a better sense of non-clinical interventions of COVID-19 locally, nationally, and internationally. At that time there was a generalized sense of fear and widespread sensationalism that was broadcast via a multitude of media. A team of 37 members of researchers in health and data sciences from the centre assembled on Slack to create a ``COVID-19 Working Group'' determined to research COVID-19 data in response to the urgent call for information. The hope was to help by contributing critical information to aid informed decision-making about managing the pandemic. Working under an immense sense of urgency, the team collected cumulative and daily case numbers, researched global COVID-19 policies, and worked on epidemiological disease models that informed the status of the pandemic on a local and national scale. This research was used by municipal and provincial policy-makers. 
Two team members promptly responded by using open COVID-19 data and a web charting library to, within a few days, assemble a website that tracked the changing local and provincial COVID-19 data. This website became known within the team as the ``COVID-19 Tracker'' ~\cite{COVIDTracker}. During the first 8 weeks, the site garnered 15,000 page views.% it would be better to give dates 'between xx and zz' - the pandemic is not necessarily over. 
% @misc{COVIDTracker,
%   author = {},
%   title = {{THE COVID-19 RESPONSE
%   How is Canada doing and what should we be doing next?
%   Centre for Health Informatics, Cumming School of Medicine, University of Calgary}},
%   year = 2020,
%   url = {https://www.chi-csm.ca/},
%   urldate = {2020-08-07}
% }

While delighted about the speed of this action, the need for a more carefully designed response was noted and a different team member assembled a smaller design team. It is this smaller group that is our design team and it is our actions in this team that we focus on. Our initial conversations in the design team were via a specifically formed Slack channel.
Our design team's dedicated channel decreased the amount of notifications to members of the COVID-19 Working Group and helped focus our discussions. 
%why
%We transitioned into a smaller design team %smaller than the 8 member?/
Additionally, our design team  started to meet using video conferencing.
We discussed COVID-19 design issues to better understand the impact of design on a broader cross-section of people.
% , not just team members but also more generally the public. %why
Our design team delved into the intricacies of the available public COVID-19 data with the goal of designing data visualizations that would support a broad cross-section of the population, which the working group had identified as important: provincial and municipal decision makers, public health officers, as well as the general public. %] %do we have an audience?
%understand the meaning of vast information about COVID-19. 
We met frequently --- often several hours a day and still met more than once a week with the COVID-19 Working Group to align with the project needs and direction in response to the status of the pandemic. %not clear


% \tatiana{We conducted a self-study for this project by integrating hermeneutic phenomenology \cite{van2016researching} and auto-ethnographic research approaches \cite{chang2013individual}. They support our scientific inquiry by deepening our understanding of the human experience as visualization designers \textit{doing} viz in a specific context. Auto-ethnographic research is befitting because its primary evidence base is the narrative of the author(s) \cite{chang2013individual}, while hermeneutic phenomenology is a suitable complement as it studies the meanings of lived experience via texts and artifacts through a creative approach of iterative self-reflection, writing, and discussion \cite{van2016researching,laverty2003hermeneutic}. Though more commonly seen in the social sciences, we benefit from these qualitative research approaches because they enable us to focus on our unique experiences of designing visualizations in a distinct context to reveal themes that occurred in non-linear collaborative practice. Provided that data visualization methods and processes are often not linear and often context specific, our research findings enrich a shared understanding of diverse socio-cultural dimensions. Our extracted themes offer an example to the members of the viz community who may identify with and acknowledge similar experiences that they too had, which serve to amplify an experiential evidence base to inform future visualization research and methodology.}


% \subsection{Our Data and Research Process}

% We developed the complexity of this visualization project through iterative analysis of our own experiential data and project artifacts \cite{creswell2016qualitative, laverty2003hermeneutic,chang2013individual}. We are the subjects providing phenomenological evidence through a self-reflexive account; we follow by evaluating our experience as a multi-disciplinary team of designers to derive meanings. We explored the following question: \emph{how has distributed video conferencing shaped our experience of synchronous design?}


% \begin{itemize} \item We collected our data – team notes in Google Docs, team's visualization sketches, design brief, and Slack history texts. We created a visual timeline from our Slack history
% \item We acknowledged our relationships that contributed to personal biases relevant to the project
% \item We wrote questions to guide our study and reflection based on our collected data and previous personal experiences relevant to visualization work and health
% \item We acknowledged and detailed our previous experience of designing visualization and how it impacted our contributions to the project
% \item We characterized, analyzed and reflected on our texts, discussed the texts, and generated new texts
% \item We held reflective discussions and documented the notes in Google Docs; themes that emerged in our text and from our reflective dialogue were grouped
% \item We interpreted our documented themes and continued to write our account
% \item We corroborated collective written experiences with one another through further discussion to validate the findings
% \item We wrote this paper detailing our experience and findings after cycling through the steps above
% \end{itemize}




%  \subsection{Our Context}
% March 13, 2020, two days before a local state of emergency was announced, the office of the mayor requested help from the Centre of Health Informatics to get more information about non-clinical interventions of COVID-19 locally, nationally, and internationally. At that time there was a generalized sense of fear and widespread sensationalism that was broadcast via a multitude of media. A team of 37 members of researchers in health and data sciences from the centre assembled on Slack determined to research COVID-19 data in response to the urgent call for information. The hope was to help by contributing critical information to aid informed decision-making about managing the pandemic. Working under an immense sense of urgency, the team collected cumulative and daily case numbers, researched global COVID-19 policies, and worked on epidemiological disease models that informed the status of the pandemic on a local and national scale. This research was used by municipal and provincial policy-makers. One team member's quick response was to make use of existing infovis templates and within a few days, they assembled a local and provincial COVID-19 data website that tracked the changing COVID-19 data, and became known within the team as the COVID-19 tracker site. This site garnered 15,000 viewers during the first 8 weeks.% it would be better to give dates 'between xx and zz' - the pandemic is not necessarily over. 
% While delighted about the speed of this action, the need for a more carefully designed response was noted and a different team member assembled a smaller design team. It is this smaller group that is our design team and it is our actions in this team that we focus on. Our initial conversations in this smaller group were via a specifically formed Slack channel but sooner moved to Zoom meetings.   
% Our stated purpose was to hold discussions about COVID-19 design issues explicitly to better understand the impact of design on a broader cross-section of people, not just team members but also more generally the public. %why
% This design team's dedicated channel decreased the amount of notifications to members not directly involved and helped focus our discussions. %why
% %We transitioned into a smaller design team %smaller than the 8 member?/
% Our design team delved into the intricacies of the available public COVID-19 data with the goal of designing data visualizations that would help as many different populations that the larger team had identified as important to inform: provincial and municipal decision makers, public health officers, as well as the public. %] %do we have an audience?
% %understand the meaning of vast information about COVID-19. 
% We started to meet frequently - often several hours a day and still met more than once a week with the larger group to align with the project needs and direction in response to the status of the pandemic. %not clear


==> [BELIV 2020] Remote COVID-19 Design/sections/30-our-design-process.tex <==
\section{Describing Our Design Process Experiences}

In this section we describe how we experienced the activities that we engaged in as the design team. In keeping with our auto-ethnographic and phenomenological methodologies, rigor in this report means staying true to the reality of our experiences in our team via detailed descriptions and iterative reflections on our texts and artifacts~\cite{laverty2003hermeneutic,creswell2016qualitative}.
In starting our distributed design process, we consulted with the literature. However, we discovered only limited advice on how to organize collaborative synchronous distributed visualization design processes. While we considered our readings about visualization design and distributed design in CSCW, we largely relied on our own, largely face-to-face, experience of prior design processes in visualization design and beyond. Here, we describe how we experienced synchronous distributed visualization design. By articulating challenges and strategies, we discuss the factors that arose in our experiences that may prove useful to consider when doing synchronous distributed visualization design.

\subsection{Establishing Meetings and Technologies} 

%Establishing the Design Team
% where and how we got inspiration: News media, Canada province responses, primary literature in vis and (public) health, other countries, anything else?
%Initially \soren{Not entirely true. At that time, D1, D5, D6 had been discussing the project for almost two weeks} the PIs discussed possible members balancing skills in data visualization, design, public health data expertise, and programming skills. D1 assembled the team and established the meeting times. 
% \tatiana{Our team of D1-D6 was working together for the first time, though some team members have worked together previously on separate projects. The team dynamics and the social setting of the lockdown were novel to the whole team. The domain specific data and the needs of the project had yet to be learned thus the team needed to get acquainted with one another as well as the data. We found that spending more time together in a synchronous setting facilitated an immediate peer-to-peer learning, and increased the ways we  communicated concurrently – in our experience, this was the most suitable way for us to connect, to build personal relationships in our group and improve group synergy. Initially, the small team of D1, D5, and D6 discussed the project for approximately two weeks. Then D1 and D2 discussed possible additional members balancing skills in data visualization, design, public health data expertise, and programming skills. D1 assembled the team and established the meeting times.}

%A callout from the Centre of Health Informatics prompted the group of researchers to band together and help with the pandemic as time was of the essence. The PI of our design team connected with collaborators with backgrounds from computer science, public health and communication, and data visualization design who were willing to join the efforts of designing COVID-19 visualizations remotely. 

% \begin{table}[tb]
% \centering
% \begin{tabular}{@{}llp{3cm}l@{}}
% \toprule
% Designer & Role         & Expertise in use                                              & Timeline %\\ \midrule
% D1       & PI           & Visualization, design, programming, management, communication & Early to late         \\
% D2       & Co-PI        & Visualization, design                                         & Late    %              \\
% D3       & Design lead  & Visualization, design                                         & Mid to %late           \\
% D4       & Designer     & Public health data expertise, design                                      & Mid to %late           \\
% D5       & Intern       & Visualization, programming                                    & Early to %mid          \\
% D6       & Intern       & Visualization, programming                                    & Early to %mid          \\ \bottomrule
% \end{tabular}
% \caption{Overview of our team.}
% I would like to make a better version of this for camera ready. I imagine you could show a column for each expertise, and then have a vertical label across the column that describes the skill
% \label{tab:overview-of-designers}
% \end{table}

% \begin{table}[tb]
% \centering
% \begin{tabular}{@{}llp{4cm}l@{}}
% \toprule
% Designer & Role         & Expertise in use                                               \\ \midrule
% D1       & PI           & Visualization, design, programming, management, communication         \\
% D2       & PI           & Visualization, design                                                  \\
% D3       & Design lead  & Visualization, design                                           \\
% D4       & Designer     & Public health data expertise, design                                         \\
% D5       & Intern       & Visualization, programming                                    \\
% D6       & Intern       & Visualization, programming                                    \\ \bottomrule
% \end{tabular}
% \caption{Overview of our team.}
% % I would like to make a better version of this for camera ready. I imagine you could show a column for each expertise, and then have a vertical label across the column that describes the skill
% \label{tab:overview-of-designers}
% \end{table}


% \subsection{Meetings}

The design team met to discuss and to sketch together for two hours a day, five days a week and attended half hour meetings with the broader team a few times per week. We mostly used Zoom~\footnote{https://zoom.com/} for meetings, Slack~\footnote{https://slack.com/} for short asynchronous communications, Google Docs~\footnote{https://docs.google.com/} for written notes and records, and Miro Board~\footnote{https://miro.com/} for collaborative design. 

Daily 2-hour meetings over Zoom brought the team together and allowed for developing an awareness of each other and established a social dynamic and rapport among the team members. The meetings were a time to convene and establish project expectations, sketch, and design together. Most of us had device cameras positioned to show our face during the Zoom meetings. The team also participated in the larger Zoom meetings with the COVID-19 Working Group to gain feedback on our visualization ideas and sketches, and to hear of new developments or requests from senior leadership. A Slack channel was the main hub to set up meeting times, to share reading and video materials about COVID-19 data and visualization design, and to inform each other of online events such as webinars. We also used the Slack channel to post our design ideas. Our visualization design team made  use of a collaborative digital whiteboard (Miro). This provided digital space for the group to post sketches, PDF’s, and virtual sticky notes during design meetings. Meeting notes and a design brief were created and stored in Google Docs and were used concurrently during our team meetings with one team member taking notes. After five weeks of daily Zoom meetings, our team reduced meeting times over a collective sense that meetings needed to be more directed and convergent — the ideation phase was wrapping up and the team was keen to implement the design. 


\subsection{Defining a Purpose and Setting a Direction}
% \cite{segel2010narrative}
% \cite{hullman2011visualization}

% In our design process, we considered literature on using storytelling elements in visualization [cite]. For example, we considered the Martini Glass structure in order to scaffold the complexity of the data and to create cohesion between COVID-19 charts to deepen an understanding of the complexity at hand. We also considered critical discussions of visualization [cite]. For example, while we were interested in helping people understand relationships between otherwise disparate datasets such as case numbers and policies, we recognized that separating certain data from the chart was critical to ensure that correlation was not assumed by the viewers such as overlaying policy data over case numbers could be misconstrued as a causal relationship.
%  In starting our distributed design process, we consulted with the literature outlined above. However, this body of literature offers limited advice for how to organize collaborative distributed visualization design processes. Instead, while considering our readings about visualization design and CSCW distributed design, we drew from our own previous experience -- largely face-to-face -- design processes in visualization design and beyond. In the following, we describe our experiences with doing distributed visualization design and then, in the next section, we offer a discussion of factors to consider through an articulation of challenges and opportunities. 

To reach a shared understanding of the project expectations, including timelines and target audiences, we collaboratively authored a design brief. This document directed some of our discussions as we considered the purpose of the site, our audience, and their familiarity with the data. The ideation process began with a distributed face-to-face critique of the COVID-19 visualizations that were already available on our site and across all of the provincial sites in Canada. 
% In addition, we identified misleading COVID-19 data visualizations on a local public health site and were able to provide feedback to its creators and remedy the situation. 
Screenshots of the various visualizations were compiled on a Miro board along with suggestions for improvements. This in turn led to ideas for improvements to the COVID Tracker website. The activity of critiquing visual elements of other visualizations was a beneficial learning exercise that focused our sketching sessions and informed our design choices. This activity enabled an engaged exploration of the data, of the end-user audience, and the purpose and messaging of the visualizations. Importantly, this activity presented the complexity of the data and enabled us to identify further questions and consultations necessary to validate our findings. While we were interested in helping people understand relationships between otherwise disparate data sets, such as case numbers and policies, we recognized that separating certain aspects of the data was critical so as to not suggest causation where correlations might exist. For example, it became clear that juxtaposing policy data with case numbers could be misconstrued as a causal relationship. 
% We subsequently validated this concern with a researcher from our COVID-19 Working Group. 



\subsection{Regular Sketching Sessions}
The goal of our synchronous online meetings during the ideation phase was to generate many ideas and sketches, while gaining an understanding of COVID-19 data. We spent a lot of time considering and exploring the data; understanding testing rates, positive case numbers, hospitalization cases, and disease transmission along with policies and correlations. We formed questions through repeated discussions, which, in consultation with members of the COVID-19 Working Group, provided a rich method for developing an in-depth understanding of the data and issues of interest. 

Sketching was a valuable activity that helped us to think through concepts, envision a story, and share ideas. Sketching enabled our team to see the data and gain a shared sense of our individual perspectives. During the meetings, and while apart, we sketched on paper and tablets. The sketches were the main artifacts that we each created and showed to each other either through presenting our physical sketch to the device camera or posting it onto our Miro board. The sketches served as the foundation for our discussions.

The design meeting notes and artifacts were stored, categorized by date, and accessible to the team. The cache of sketches along with inspiration clippings and meeting notes proved very useful. We were able to refer to previously posted resources and sketches during design meetings, enhancing our ability to recall our previous work and build on it. However, we found the lag time when posting our paper sketches onto our virtual whiteboard to be challenging. We dealt with this by holding sketches up to the camera, but they were not easily referenced until they were scanned and added to the board.

%as references to our ideas during the ideation phase.
% Showing sketches over teleconferencing does not work with virtual backgrounds. %can you say more about this?

\subsection{Software Prototyping}
Illustrator versions of our design were produced by the lead designer so we could view a pixel-perfect design. After several iterations, the Illustrator file was handed off to three team members who implemented the design using D3~\cite{bostock2011d3}. Several iterations of the software prototype were critiqued during collaborative design team sessions and subsequently tweaked. The design phase for the data visualization continued through implementation as updating data sources presents new challenges to be solved. When prototypes were polished and reflected live data sources, they were presented in a Zoom meeting to the COVID-19 Working Group for feedback. 



==> [BELIV 2020] Remote COVID-19 Design/sections/35-defining-our-needs-as-designers.tex <==
%\subsection{Identifying Missing Factors}
%% this strikes me as more what I would see being in section 3
%We, as designers, needed to think critically about how to tell the story with the data as a way to communicate the complexity of the pandemic in the interest of ensuring that our visualisation would not be misinforming. In order to support the process of ideation and data discovery, we wished to collaborate via a real-time sketching setup similar to collocated design environment such as a lab. The familiar lab environment facilitated serendipity, natural discussion and a tangible sense of togetherness that allowed for ideas to spontaneously emerge.  Therefore, we pursued to create a real-time collaborative sketching experience while being in disparate geographical locations. We searched for useful tools and materials to enable the team members to communicate ideas about interactions for the design and to share them, as we normally would, ‘in-person’. 

%\section{Defining Our Needs as Designers}
%% this strikes me as more what I would see being in section 3
%We, as designers, needed to think critically about how to tell the story with the data as a way to communicate the complexity of the pandemic in the interest of ensuring that our visualisation would not be misinforming. In order to support the process of ideation and data discovery, we wished to collaborate via a real-time sketching setup similar to collocated design environment such as a lab.  The familiar lab environment facilitates serendipity, natural discussion and a tangible sense of togetherness that allows for ideas to spontaneously emerge.  Therefore, we pursued to create a real-time collaborative sketching experience while being in disparate geographical locations. We searched for befitting tools and materials available to enable the team members to communicate ideas about interactions for the design and to share them, as we normally would, ‘in-person’. 


==> [BELIV 2020] Remote COVID-19 Design/sections/40-challenges.tex <==
\section{Emerging Factors in Our Virtual Visualization Design}
Our purpose was to think critically about how to communicate the complexity of the pandemic and the data while ensuring that our visualization would not be misinforming. Our process, however, started by identifying the missing factors in our distributed design situation. The familiar lab environment facilitated serendipity, natural discussion, and a tangible sense of togetherness that allowed for ideas to spontaneously emerge. In order to support the process of ideation and data discovery in our distributed environment, we wished to collaborate via real-time sketching and discussion akin to a collocated design environment such as a lab. We searched for useful tools and materials to enable the team members to communicate ideas about interactions for the design and to share them, as we normally would, ``in-person''. 

We note that being distributed forced us to be upfront about the process. This in turn supported later reflection because our distributed work had been logged through the various tools used in the design process. This design experience was distinct as a result of distributed collaboration under the time sensitive demands of a public health emergency. Furthermore, remoteness posed a perceived risk of misunderstanding and miscommunication, more so given a flux of ever-changing public health data that decision makers were relying upon. This design experience elucidated several factors for re-consideration. Notably, these factors were initially experienced as challenges but sometimes, through working with these challenges, we also noted potential strategies and opportunities. 
%While doing distributed visualization design posed challenging as we have described above, this mode of working also provided opportunities. Here, we outline 
% We recognize that some of the experiences we describe seem to as easy, or potentially easier than co-located design work. 

%\fix{x} \textbf{
In the following, we describe eleven factors that emerged from an auto-ethnographic exploration of our distributed visualization design process. While the design factors encompass a wide array of considerations, we recognize that there are more opportunities and strategies possible through re-purposing current software and hardware tools. 
% We just mention the ones that we tried.
%\challengesection{C0. Prototypical challenge}
%\textit{Briefly (2-4 lines), What is the challenge}
%Longer explanation of why this challenge is important to be aware of.
%For example, \ldots
%Reflecting on the challenge
%(possibilities/or what we did to solve it).
%\challengesection{C1. Barrier to ‘face-to-face’ communication}
 \subsection{Pandemic Challenges}
 
%Our first challenge is specific to the situation during the COVID-19 pandemic lockdown. 
First and unsurprisingly, the pandemic lockdown led to challenges. These are important to recognise as they heavily influenced our ability to carry out work.
 
 \challengesection{C1. Negotiating Time and Resources}
\textit {Coordinating time and access to physical space for some team members was a challenge amidst the social lockdown. This challenge is important because the pandemic brought forward some social constraints to distributed work from home such as interruptions in each member’s home environment, lack of physical working space, and faulty hardware that played a role in how the team managed to design together remotely.} 
For example, some collaborators were forced to leave meetings in order to take care of their children and at times their children showed themselves to the camera during design meetings. There were instances when team members had to move their device to a different room during meetings because their small shared living spaces were prioritized based on homeschooling needs of children or for other family members who were working from home. We contended with web cams that did not function, so some team members were not visible during camera-to-camera meetings. Purchasing web cameras at the time was difficult due to a high demand in the market with increased remote work. As a team, we resolved to continue meetings during these circumstances. Audio was muted for a moment when children interrupted our online meetings and we waited until family disruption ended. We persisted with meetings though some members were not visible, interacting only via audio.
Additionally, this work provided an opportunity to ``be with'' other people and to ``contribute'' in a way that was a cathartic exercise for several team members in the midst of this pandemic.

 \section{Communication Breakdowns}
 
 This group of challenges focus on how our adaptation to distributed collaborations caused several types of communication challenges — some of which we learned how to mitigate.
 
\challengesection{C2. Establishing Team Cohesion}
\textit {The sense of uncertainty that arose steeply during the initial COVID-19 lockdown, along with our own perceived challenges of remote collaboration, posed risks of miscommunication and possible difficulties in establishing a spirit of team trust and cohesion.}
This was a challenge we were particularly aware of, because, while most of us were in the same geographical region, we designed synchronously from our homes. Our intention was to recreate the familiar ``face-to-face'' co-located communication flow even though we were working in a distributed virtual setting.
We chose frequent synchronous virtual collaboration as a way to 1) align our ideas and learn 2) mitigate a sense of uncertainty during a pandemic with frequent feedback 3) establish team cohesion and rapport. 
This virtual space was a new reality for many collaborators.
% due to the pandemic. 
Seeing one another brought a sense of togetherness and co-presence that was conducive to successful and natural synchronous teamwork. Notably, it was possible for our virtual interaction to achieve a similar communication workflow with the team’s facial expressions and gestures visible through our device cameras. Human communication and connections are an interplay of nuanced cultural mannerisms that may not be visible or as obvious through a webcam. Nonetheless, seeing each other through webcams and computer screens established a collective awareness and a sense of attendance within the team though we were not co-located. However, eye-to-eye contact differed from being co-located. We tended to look at each other's faces on the screen and not directly into our cameras, often seeming as though eye contact was averted during conversations. We found that group etiquette naturally developed in our online work space such as muting the microphone during excessive background noise, putting up a hand to speak, and waving goodbye into the camera. 
A couple of the team members chose to keep their cameras off during all online meetings but remained audible, which created a barrier to gaining an understanding of their affect and their level of engagement because gestures, facial expressions, and eye contact were not visible. We found that members who had their cameras turned on often dominated and contributed more to the discussion and invested more time throughout the project.
% \challengesection{C5. Creating a Team Working Space}

  \challengesection{C3. Understanding Team Members' Progress}
\textit {The challenge was to determine the progress of individuals on the team so that we could move forward with project goals. It was important to understand where team members were in their work to ensure that we were completing our goals.}
The team was rapidly assembled; some members were volunteers. They were unfamiliar with each other’s skills and were unsure if it was okay to ask others given the circumstances. Some work needed to be done asynchronously and, from time to time, team members were not able to follow through with tasks.
For example, we decided to assign tasks such as to scope nationwide provincial sites for visualizations of COVID-19 data and compile the findings in an Excel file, while another member was reviewing other information outside of our team meetings.
It was also valuable to prepare some information before our design team meetings to bolster our discussions about visualization design. To ensure that everyone was aware of the status of each task, team member A would check on the progress via Slack, which was visible to the whole team. This method was useful to ensure transparency and clear expectations for individual task completion within our design process. 
Some members, notably team members C and D often self-assigned tasks while other members relied upon A for task assignment and review.
 
 \challengesection{C4. Diversity of Software and Sketching Expertise}
\textit {There was considerable variation in levels of skill when sketching ideas or visualizing data, meaning that some of the team members struggled more than others with design activities and required guidance.} 
As a solution to some of these differences, the lead visualization designer mentored willing team members who were less experienced in designing data visualizations. For example, we held optional group sketching sessions via Zoom as a way to learn and to practice sketching apart from our team meetings. To bypass software knowledge gaps, we photographed physical paper sketches and shared them on the Miro board because everyone was able to use their device cameras comfortably. However, photographing our sketches stifled the natural flow of sketching and sharing during meetings, so we reverted to sketching and presenting our sketches through the camera. This method led to more productive discussions and more sketching to take place during the meetings.
We also saw a benefit in the virtual environment because sketches could be easily seen by everyone at the same time provided the camera was set up in such a way that the sketch was well lit and in focus. We would often scan sketches using a phone app or transfer them to the digital whiteboard, where we could continue to review the sketches.
After reviewing the sketches and discussing their features we decided on the best sketch to prototype. 
We also found screen sharing to be a benefit during the polishing stage of a working prototype. While designers might want to adjust some of the positioning and style of elements in a working prototype, they may not have a development space set up or the skills to make those adjustments. The programming team members utilized screen sharing to collaboratively make those adjustments in real time with the designers.
 
% \begin{figure*}[tb!]
%   \centering
%   \includegraphics[width=\textwidth]{figures/inspiration-cropped2.png}
%   \caption{An excerpt of our Miro board. In this area of the board, we compiled COVID-19 visualisations for shared inspiration, data understanding, and critique. We continually referred back to this area of the board during our design sessions.}%\soren{This can't be empty. Also, we need higher resolution}.}
%   \label{fig:inspiration-board}
% \end{figure*}
%  \subsection{Visualization Design Process}
  
 % This section discusses factors that arose throughout our design process.
  
\challengesection{C5. Understanding and Sharing Data}
\textit {Learning about the project needs and the health data was foundational to our visualization design, so we spent considerable time reviewing and discussing policy data, testing data, health care system capacity, social determinants of health, studying COVID-19 visualizations across Canadian jurisdictions, and in regular consultations with the COVID-19 Working Group in a remote setting.} 
As COVID-19 data was being visualized broadly across the world, we knew how the data was typically shown, so we considered the clarity and lack of clarity in existing visualizations. Therefore, we looked for new ways to visualize the same data that would not perpetuate the same issues. Information gathering was crucial to our design process because it enabled us to identify relationships and assumptions within the data as we sketched data visualizations in the early design stage. Notably, this process provided a fruitful distributed design environment with a serendipitous sense of data discovery. This collaborative online knowledge seeking provided a generative online learning space. Additionally, this activity allowed us to deepen our collective understanding of the data and cultivated team rapport.
This is an area where we identified a clear benefit to working in a distributed environment. We were able to work independently and then quickly share our findings when identifying something interesting. For example, we considered critical discussions of visualization, such as the understanding that positive cases were indicative of testing capacity. We followed this insight by brainstorming ways to visualize this relationship in a more clear manner as part of a larger visualization product. 
 % fill if possible ~\cite{} while reviewing the data with a sense of urgency; an extended amount of time was spent exploring the data and communication to the audiences with a heightened sense of risk if the data were misrepresented in our design. The activity of critiquing visual elements of other visualizations was a beneficial learning exercise that sparked productive questions and rich discussions.
\challengesection{C6. Sharing and Acquiring Knowledge}
\textit{It was challenging to share and introduce knowledge and background skills to other team members. Likewise, it was challenging to acquire new understanding from other team members.}
Distributed modes of collaboration introduce more friction in sharing knowledge. It is more difficult to find and share resources and point to specific parts of a resource as it is prone to error and requires time. This is particularly relevant in a visualization context. In contrast, in co-located situations pointing, body language, and using artifacts such as laptops to communicate ``see this'' is easy and affords a low-friction possibility for understanding whether you have caught peoples' attention. In extension, these situations allow the receiving side to see exactly what is meant and allow for clarifying questions to a specific aspect. 
For example, we discussed story-telling aspects of our design. However, discovering the depth and subtlety of the data and how it fits with storytelling concepts appeared overwhelming. Especially as we intended to deepen a shared understanding of this data through visualizations and storytelling, and further, from an interaction perspective, to use scrollytelling to show the complexity of COVID-19 data.
We considered literature on using storytelling elements in visualization~\cite{riche2018data} to prompt meaningful discussions about the data. For example, we referred to the Martini Glass structure~\cite{segel2010narrative} as a potential way to scaffold the complexity of the data and to create cohesion between COVID-19 charts. However, while all team members attempted to grasp these concepts, some team members had a sense of superficially understanding these ideas and found it difficult to use them when thinking about designs.
Despite these challenges, working remotely also poses benefits for knowledge exchange. By working in a distributed team, resources will typically be shared through a medium that allows people to return to them, which is particularly beneficial when acquiring new knowledge.
%\newpage
\challengesection{C7. Understanding Design Ideas} 
%  One of the challenges of collaboration increases the difficulty , it is 
% serendipitous meetings, sharing physical artifacts/sketches
\textit{Working in a distributed design team adds friction to the process of understanding other collaborator’s perspective throughout the design process~\cite{gutwin1998design}. In our case, it took more time to establish understanding when sharing diverse ideas in the process of interpreting domain-specific data and creating data visualizations.}
Typically, a co-located physical space that facilitates the sharing of ideas through face-to-face team activities is used during ideation and iteration phases of the design process. For example, we would compile our sketches on the wall of a meeting room for all members to view and discuss. We adapted this activity to our online synchronous setting by posting sketches to an online collaborative whiteboard in Miro while simultaneously meeting via Zoom. Despite the learning curve of adopting the software, we found this strategy allowed us to share and discuss our ideas productively. Working in the virtual whiteboard environment opened up new opportunities that would not be as feasible when working with the physical counterpart. 
Endless space offered in the virtual whiteboard allowed the team a great deal of flexibility in how the content was laid out. Items on the board could be arranged linearly, and grouped and regrouped as the design process unfolded. The team was able to quickly reference previously shared content, which aided in clarifying how assumptions and misunderstanding had arisen. 
The ability to use virtual pointing and to jump to another's pointing location played a beneficial role in the virtual work space. While pointing is possible in the physical environment, this can at times lack accuracy or require people to physically move closer to the item they are pointing at, which is time-consuming and may occlude it. There is also the limitation that only so many people can be close to a small clipping or sketchbook page. The virtual space permits all collaborators to have an optimal view of where the speaker is pointing and an equal opportunity to point at things.
Iteration was an integral part of the design process, and for this it was often useful to markup existing sketches and design outputs. The digital environment offered the ability to quickly duplicate and markup as many copies of something as needed without compromising the integrity of the original. This was especially enabling when one team member wanted to iterate on another team member's sketch because doing so was immediate and essentially risk-free. %}
   
\section{Strategies for Distributed Design}
   
The intensity of the pandemic situation coupled with the team's general willingness to experiment led us to explore alternative uses of hardware and software. Next, we discuss current potential strategies and potential opportunities that lie ahead. 
\begin{figure*}[tb!]
  \centering
  \includegraphics[width=\linewidth]{figures/Miro_Capture.jpg}
  \caption{An excerpt of our Miro board that captures a design session for lo-fi prototyping of visualization interaction. During the session all participants were able to duplicate and arrange assets to mimic paper prototyping.}
  \label{fig:prototyping-interactions-in-miro}
\end{figure*}
% \challengesection{C6. Coordinating information about the pandemic}
% This seems irrelevant for the focus of this paper (distributed vis design)
% How the pandemic affected our ability to work. Our experience of working through the pandemic of before and after. Funding, high-level decisions the future of the project.
 
\challengesection{S1. Simulating a Co-located Design Space for Sketching}
\label{subsubsec:simulating-colocation}
\textit {It is difficult to gain a full view of group sketching in a distributed setting because online meetings are generally limited to one view per participant. In an attempt to create a real-time collaborative sketching experience, two team members tested a setup of two device cameras per person during a Zoom meeting.} 
The setup included signing into the meeting twice with two separate devices; one device was a PC camera aimed at the face of each participant and a second device was a phone camera that was directed on their paper and pen. Though it was awkward to find a suitable angle and stabilize the phone, facial expressions, gestures and gaze were captured along with a view of real time sketching. This method allowed the conversation to be held concurrently with a view of sketching practice as it was unfolding within the discussion. This remote sketching activity was seamless in a virtual distributed design setup that simulated a co-located design environment. It supported conversational and visual communication, however, it was cumbersome to recreate this physical setup and it was not attempted after a single trial.
There is considerable potential for developing better and easier ways to set up this type of distributed collaboration. For instance, this approach could bypass knowledge gaps or inaccessibility to using digital sketching tools such as a Wacom tablet. Likewise, we imagine specialised software might provide support for this purpose.
% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=\columnwidth]{figures/sticky-notes-wall-miro2.png}
%   \caption{This is an example of learning in progress. One designer reverted to a physical wall to gather their ideas on stickies, snap a photo and brought it into the Miro board (left). As a group, we wanted the re-positioning freedom of miro board stickies and remade made them to achieve this (right).}
%   \label{fig:sticky-notes}
% \end{figure}
%\challengesection{C12. Testing Design Interactions}
\challengesection{S2. Screen-Sharing to Collaborate in Software Applications}
\textit {Different team members can use their software fluency and bring different skills to the table. With the goal of including everyone throughout the design process, we used screen-sharing via Zoom to collaborate in specialized environments such as designing in Adobe Illustrator or editing code.} 
What made this method particularly useful was when there was skill cross-over in the team because meeting participants could control the mouse during a screen-sharing session. For example, a team member shared their design on the screen of an open Adobe Illustrator workspace during the Zoom meeting. Another team member controlled the mouse from a separate location on their shared Adobe Illustrator workspace. This process allowed for real-time manipulation of visual components of our design and to share skills between multiple team members.
Even in cases where collaborators were not manipulating the software remotely, we found sharing specialized environments to be useful as it mimicked casual co-located collaboration. For example, designers might often gather around the work space of the person implementing a design to tweak position, padding, and other style details. We simulated this experience with screen-sharing and being able to grant remote access to the mouse meant that team members could point out these details with accuracy. 

\challengesection{S3. Using Hand Gestures for Discussing Interaction}
\textit {Animating designs using video or animation software is difficult for team members that lack such technical skills. Not everyone in the group knew how to digitally animate a design, which excluded some team members.}
We discovered that the most accessible way for each team member to show their ideas was by talking camera-to-camera similar to a face-to-face co-located setting. The software knowledge gap was resolved by relying on hand gestures and moving static design artifacts with our hands while remaining visible in the camera. Everyone in the team with access to a web camera could speak to their ideas and show how they imagined the design would move with intuitive hand motions, facial expressions, sounds, pointing to, or moving their own sketches or cut outs while explaining their idea in front of the camera. This emphasized a fuller presence within a remote collaborative experience similar to that of a lab.
We reflected on our choice of communicating about interactions and compared it to our previous visualization design experiences. Based on this, we think we would have pointed to sketches in a co-located mode of collaboration instead of moving our hands in mid-air in front of the camera. We see the hand gestures as adding an extra barrier to communicating about interactions. 
% and assisted showing sketches over teleconferencing. We do note that showing sketches over teleconferencing does not work with virtual backgrounds. % capture diverse ideas. 
% \challengesection{C12. Moving Static Components on a Miro board}
\challengesection{S4. Lo-fi Prototyping for Visualization Interaction}
\textit {It was challenging to find optimal tools to enable all of us to test interactions in a digital format given our variable programming expertise. We aimed to re-create the use of paper prototyping in a digital format.}
To set this up, we used a digital whiteboard in Miro as a ``table top'' space and exported assets from Illustrator to use as ``paper'' clippings. Teleconferencing via Zoom enabled gesturing and speaking into the camera, while all team members could simultaneously copy, resize, and rearrange assets in Miro. Team members were able to collaboratively create UI mock-ups (Figure \ref{fig:prototyping-interactions-in-miro}) and animate them by clicking and dragging. We found this method to be quick and inclusive to all members, regardless of skill. Additionally, we found the ability to duplicate elements and groups of elements without disrupting the integrity of previous models provided a benefit over traditional paper prototyping.
% While doing distributed visualization design posed challenging as we have described above, this mode of working also provided opportunities. Here, we outline experiences that either seemed as easy, or potentially easier than co-located design work. 
% Being distributed forces you to be upfront about the process, and allow for later reflection because distributed work creates a repository
% \opportunitysection{O1. Sharing design inspiration}
% \opportunitysection{O2. Managing design artifacts}
% The design meeting notes and artifacts were stored, categorized by date, and accessible in the software that we used. This cache of meeting notes and artifacts has proved to be simple and very useful when referring to previously posted resources or sketches during design meetings, especially for recalling what we did earlier and building upon our ideas.  For example, our sketches or national COVID-19 visualizations and meetings notes were Google Docs, Slack, or Miro that are invaluable to this paper because it allowed us to reflect on our record of detailed design activities enabling more insight to occur. 
% \opportunitysection{O3. Keeping tabs on design provenance}
% How the design came to be. Data about how we worked (Zoom data, Miro board history)


%  \section{Emerging Factors for Distributed Visualization Design: Challenges and Opportunities}
% This design experience was different as a result of distributed collaboration under the time sensitive demands of a public health emergency. Remoteness posed a perceived risk of misunderstanding and miscommunication, more so given a flux of ever-changing public health data that decision makers were relying upon. Based on our design experience and reflection, several factors arose that needed re-consideration. Notably, these factors were initially experienced as challenges but sometimes, through working with these challenges, we also noted opportunities. 
% %While doing distributed visualization design posed challenging as we have described above, this mode of working also provided opportunities. Here, we outline 
% % We recognize that some of the experiences we describe seem to as easy, or potentially easier than co-located design work. 
% We note that being distributed forced us to be upfront about the process. This in turn allowed for later reflection because our distributed work created a repository.
% %\fix{x} \textbf{

% In the following, we describe eleven emerging factors for doing distributed visualization design. We present these factors in four groups: pandemic challenges, communication breakdowns, visualization design process, and strategies for distributed design. While the design factors encompass a wide array of considerations, we recognize that do not view these think that there are more opportunities and strategies possible through re-purposing current software and hardware tools. 
% % We just mention the ones that we tried.



% %\challengesection{C0. Prototypical challenge}
% %\textit{Briefly (2-4 lines), What is the challenge}

% %Longer explanation of why this challenge is important to be aware of.

% %For example, \ldots

% %Reflecting on the challenge

% %(possibilities/or what we did to solve it).

% %\challengesection{C1. Barrier to ‘face-to-face’ communication}

%  \subsection{Pandemic Challenges}
 
% Our first challenge relate specifically to the situation that was happening during the COVID-19 pandemic lockdown. 
 
%  \challengesection{C1. Negotiating Time and Resources}
% \textit {Coordinating time and access to physical space for some team members was a challenge amidst the social lockdown. This challenge is important because the pandemic brought forward some social constraints to distributed work from home such as interruptions in each member’s home environment, lack of physical working space, and faulty hardware that played a role in how the team managed to design together remotely.} 

% For example, some collaborators were forced to leave meetings in order to take care of their children and at times their children showed themselves to the camera during design meetings. There were instances when team members  had to move their device to a different room during meetings because their small shared living spaces were prioritized based on homeschooling needs of children or for other family members who were also working from home. We also contended with web cams that did not function, so some team members were not visible during camera-to-camera meetings. Purchasing web cameras at the time was difficult due to a high demand in the market with increased remote work. As a team, we resolved to continuing meetings in light of these circumstances such as when children would show up in our online meetings then audio was muted for a moment and we waited until we could return to the meeting without family interruptions. We persisted with meetings though some members were not visible, and we used audio only to interact.

% We do note that the challenges mentioned in this section are particularly pandemic related, rather than broadly related to remote working. Thus while we do feel that these challenges are important to note, they may generalize less than the other points in this section. There are a few other pandemic related factors such as the fact that this project took place quickly without time for establishing funding -- thus many team members were volunteering their time so it was difficult to assess expectations. We also note that this work provided an opportunity to "be with" other people and to "contribute" in a manner that was a cathartic exercise for some of the team in the midst of this pandemic.

%  \subsection{Communication Breakdowns}
 
%  This group of three challenges focus on how our sudden change to distributed collaborations caused several different types of communication challenges, some of which we were able to learn how to mitigate. 

% \challengesection{C2. Establishing Team Cohesion}
% \textit {The sense of uncertainty that arose steeply during the initial COVID-19 lockdown, along with our own perceived challenges with remote collaboration, made us think about risks of miscommunication and possible difficulties in establishing a spirit of team trust and cohesion.}

% This was a challenge we were particularly aware of because, while most of us were in the same geographical region, we had to do distributed design from our homes. Our intention was to recreate the familiar ‘face-to-face’ co-located communication flow even though we were working in a distributed virtual setting. As a way to mitigate the risk of miscommunication as we aligned our ideas, we opted for long daily virtual face-to-face collaboration. Most of the team met at least 2 hours per day, with some sub-groups extending this virtual face-to-face time. We emphasize our responses to the challenges that relate to this mode of collaboration.
% We chose frequent synchronous virtual collaboration as a way to 1) align our ideas 2) mitigate a sense of uncertainty during a pandemic with frequent feedback 3) establish team cohesion and rapport. 

% Importantly, human communication and connections are an interplay of nuanced cultural mannerisms that may not be visible or as obvious through a webcam. We found that group etiquette naturally developed in our online work space such as muting the microphone during too much background noise, putting up a hand to speak, and waving goodbye into the camera. 

% This virtual space was a new reality for many collaborations due to the pandemic. Seeing one another brought a sense of togetherness and co-presence that was conducive to successful and natural synchronous teamwork. Notably, it was possible for our virtual interaction to achieve a similar communication workflow with the team’s facial expressions and gestures visible through our device cameras. Seeing each other through webcams and computer screens established a collective awareness and a sense of attendance within the team though we weren't co-located. However, eye-to-eye contact differed from being co-located. We tended to look at each other's faces on the screen and not directly into our cameras, often seeming as though eye contact was averted during conversations. A couple of the team members chose to keep their cameras off during all online meetings but remained audible, which created a barrier to gaining an understanding of their affect and their level of engagement because gestures, facial expressions, and eye contact were not visible. We found that members who had their cameras turned on often dominated the discussion and contributed more to the discussions and invested more time throughout the project.

% % \challengesection{C5. Creating a Team Working Space}

% %\textit {The sense of uncertainty that arose steeply during the initial COVID-19 lockdown, along with our own perceived challenges with remote collaboration, made us think about risks of miscommunication and possible difficulties in establishing a spirit of team trust and cohesion.} 

% %This was a challenge we were particularly aware of because, while most of us were in the same geographical region, we had to do distributed design from our homes. Our intention was to, as best possible, recreate the familiar ‘face-to-face’ co-located communication flow even though we were working in a distributed situation and our 'face-to-face' was virtual only. However, to mitigate the risk of miscommunication as we aligned our ideas, we opted for long daily virtual face-to-face collaboration. Most of the team met at least 2 hours per day, with some sub-groups extending this virtual face-to-face time. 
% %, we emphasize our responses to the challenges that relate to this mode of collaboration.
% %We chose frequent synchronous virtual collaboration as a way to 1) align our ideas 2) mitigate a sense of uncertainty during a pandemic with frequent feedback 3) establish team cohesion and rapport. 

% %This virtual space is a new reality for many collaborations due to the pandemic. Seeing one another brought a sense of togetherness and co-presence that was conducive to successful and natural synchronous teamwork. Notably, it was possible for our virtual interaction to achieve a similar communication workflow with the team’s facial expressions and gestures visible through our device cameras. Seeing each other through webcams and computer screens established a collective awareness and a sense of attendance within the team though we were in separate geographic locations. Conversely, a couple of the team members chose to keep their cameras off during all online meetings but remained audible, which created a barrier to gaining an understanding of their affect and their level of engagement as gestures and eye contact were not visible. Notably, the members who had their cameras turned on often dominated the discussion and ultimately contributed more time and conversation throughout the project.



%   \challengesection{C3. Understanding Team Members' Progress}
% \textit {The challenge was to determine the progress of individuals on the team so that we could move forward with project goals. It was important to understand where team members were in their work to ensure that we were moving along as a cohesive team.}

% The team was assembled rapidly and mostly as volunteers, individuals either were not always aware of each others skills and/or were not sure what was okay to ask of others given the circumstances. 
% Some work need to be done asynchronously and, from time to time, team members might not be able to follow through with these tasks.
% For example, we decided to assign tasks such as scope nationwide provincial sites for visualizations of COVID-19 data and compile the findings in an Excel file, while another member was reviewing other information outside of our team meetings.
% It was valuable to have some information prepared before our design team meetings to bolster our discussions about visualization design. To ensure that everyone was aware of the status of each task, the P1 would check on the progress via Slack that was visible to the whole team. This method was useful to ensure transparency and clear expectations for individual task completion within our design process. 
% Some members, notably P3 and P4 often self-assigned tasks while other members relied upon P1 for task assignment and review.
 
%  \challengesection{C4. Diversity of Software and Sketching Expertise}
% \textit {There was considerable variation in levels of skill  when sketching ideas or visualizing data, meaning that some of the team members struggled more than others with  design activities and required guidance.} 

% As a solution to some of these differences, the lead visualization designer mentored willing team members that were less experienced in data visualization design. For example, we held optional group sketching sessions via Zoom as a way to learn and to practice sketching apart from our team meetings. To bypass software knowledge gaps, we photographed physical paper sketches and shared them on the Miro board because everyone was able to use their device cameras comfortably. However, photographing our sketches stifled the natural flow of sketching and sharing during meetings, so we sketched and presented our sketches through the camera. This method enabled productive discussions and more sketches to take place during the meetings.

% We also here saw a benefit in the virtual environment because sketches could be easily seen by everyone at the same time provided the camera was set up in such a way that the sketch was well lit and in focus. We would often then scan sketches using a phone app or transfer them if drawn on a tablet to the digital whiteboard, where we would continue to review the sketches.
% After reviewing the sketches and discussing their features we decided on the best sketch to prototype. 

% We also found screen sharing to be a benefit during the polishing stage of a working prototype. While designers might want to adjust some of the positioning and style of elements in a working prototype, they may not have a development space set up or the skills to make those adjustments. The team member writing code utilized screen sharing to collaboratively make those adjustments in real time with the designers.
 
% \begin{figure*}[tb!]
%   \centering
%   \includegraphics[width=\textwidth]{figures/inspiration-cropped2.png}
%   \caption{An excerpt of our Miro board. In this area of the board, we compiled COVID-19 visualisations for shared inspiration, data understanding, and critique. We continually referred back to this area of the board during our design sessions.}%\soren{This can't be empty. Also, we need higher resolution}.}
%   \label{fig:inspiration-board}
% \end{figure*}


%  \subsection{Visualization Design Process}
  
%   This section discusses factors that arose throughout our design process.
  

% \challengesection{C5. Understanding and Sharing Data}

% \textit {Learning about the project needs and the health data was foundational to our visualization design, so we spent considerable time reviewing and discussing policy data, testing data, health care system capacity, social determinants of health, and as well as studying COVID-19 visualizations across Canadian jurisdictions, along with holding regular consultations with the larger group of researchers on our team in a remote setting.} 

% As COVID-19 data was being visualized  broadly across the world, we knew how the data was typically shown, so we considered the clarity, and lack of clarity in existing visualizations and looked for new ways to visualize the same data that might not perpetuate the same issues. Information gathering was crucial to our design process because it enabled us to identify relationships and assumptions within the data as we sketched data visualizations in the early design stage. Notably, this process provided a fruitful distributed design environment with a serendipitous sense of data discovery. This collaborative online knowledge seeking and sharing provided a generative online peer-to-peer learning space and was a meaningful activity for us to deepen our collective understanding of the data and cultivate team rapport and cohesion.
% This is an area where we identified a clear benefit to working in the virtual environment, because we were able to work independently and then quickly share our screens if something interesting was found. For example, we identified that positive cases were indicative of testing capacity so we brainstormed about a way to visualize this relationship in a more obvious way as part of the whole story. 

% We also considered critical discussions of visualization % fill if possible ~\cite{} 
% while reviewing the data with a sense of urgency; an extended amount of time was spent exploring the data and communication to the audiences with a heightened sense of risk if the data were misrepresented in our design. The activity of critiquing visual elements of other visualizations was a beneficial learning exercise that sparked productive questions and rich discussions.

% \challengesection{C6. Sharing and Acquiring Knowledge}
% \textit{It is challenging to share and introduce knowledge and background skills to other team members. Likewise, it is challenging to acquire new understanding from other team members.}

% Distributed modes of collaboration introduce more friction in sharing knowledge. It is more difficult to find and share resources, and to point to specific parts of a resource is more labor intensive and prone to error. This is particularly relevant in a visualization context. In contrast, in co-located situations pointing, body language, and using artifacts such as laptops to communicate ``see this'' is easy and affords a low-friction possibility for understanding whether you have caught peoples' attention. In extension, these situations allow the receiving side to see exactly what is meant and allow for clarifying questions to a specific aspect. 

% For example, we discussed story-telling aspects of our design. However, discovering the depth and subtlety of the data and how it fits with storytelling concepts appeared overwhelming. Especially as we intended to deepen a shared understanding of this data through visualizations and storytelling --- and from an interactive perspective, using `scrolly-telling' --- to show the complexity of COVID-19 data.
% We considered literature on using storytelling elements in visualization~\cite{riche2018data} to prompt meaningful discussions about the data. For example, we referred to the Martini Glass structure~\cite{segel2010narrative} as a potential way to scaffold the complexity of the data and to create cohesion between COVID-19 charts. However, while all team members attempted to grasp these concepts, part of the team had a sense of superficially understanding these ideas and found it difficult to use them when thinking about designs.

% Despite these challenges, working remotely also poses benefits for knowledge exchange. By working in a distributed team, resources will typically be shared through a medium that allows people to come back to it later, which is primarily beneficial when acquiring new knowledge.
% \newpage
% \challengesection{C7. Understanding Design Ideas} 
% %  One of the challenges of collaboration increases the difficulty , it is 
% % serendipitous meetings, sharing physical artifacts/sketches
% \textit{Working in a distributed design team adds friction to the process of  understanding other collaborator’s perspective throughout the design process~\cite{gutwin1998design}. Specifically in our case, it took more time to establish understanding when sharing diverse ideas in the process of interpreting domain-specific data and creating data visualizations.}

% Typically, a co-located physical space that facilitates the sharing of ideas through face-to-face team activities is used during ideation and iteration phases of the design process. For example, we would compile our sketches on the wall of a meeting room for all members to view and discuss. We adapted this activity to an our online synchronous setting by posting sketches in the online collaborative whiteboard tool (Miro) while simultaneously teleconferencing (Zoom). Despite the learning curve of adopting the software we found this strategy allowed us to share and discuss our ideas productively. Working in the virtual whiteboard environment even opened up new opportunities that would not be as feasible when working with the physical counterpart. 

% Endless space offered in the virtual whiteboard allowed the team a great deal of flexibility in how the content was laid out. Items on the board could be arranged linearly, grouped and regrouped as the design process unfolded. The team was able to quickly reference previously shared content which aided in clarifying how assumptions and misunderstanding had arisen. 

% The ability to use of virtual pointing and the ability to jump to another's pointing location was also significant. Thus pointing played a beneficial role in the virtual work space. While pointing is possible in the physical environment, this can at times lack accuracy or require the individual to physically move closer to the item they are pointing at, which is time consuming and may occlude it. There is also the limitation that only so many people can be close to a small clipping or sketchbook page. The virtual space permits all collaborators to have an optimal view of where the speaker is pointing and an equal opportunity to point at things.

% Iteration was an integral part of the design process, and for this it was often useful to markup existing sketches and design outputs. The digital environment offered the ability to quickly duplicate and markup as many copies of something without compromising the integrity of the original. This was especially enabling when one team member wanted to iterate on another team member's sketch because doing so was immediate and essentially risk-free. %}


   
% \subsection{Strategies for Distributed Design}
   
% The intensity of the situation coupled with the team's general willingness to experiment led us to explore alternative uses of hardware and software. We think that future opportunities along these lines are plentiful. 

% \begin{figure*}[tb!]
%   \centering
%   \includegraphics[width=\linewidth]{figures/Miro_Capture.jpg}
%   \caption{An excerpt of our Miro board that captures a design session for lo-fi prototyping of visualization interaction. During the session all participants were able to duplicate and arrange assets to mimic paper prototyping}
%   \label{fig:prototyping-interactions-in-miro}
% \end{figure*}

% % \challengesection{C6. Coordinating information about the pandemic}
% % This seems irrelevant for the focus of this paper (distributed vis design)
% % How the pandemic affected our ability to work. Our experience of working through the pandemic of before and after. Funding, high-level decisions the future of the project.


 



% \challengesection{C8. Simulating a Co-located Design Space for Sketching}
% \label{subsubsec:simulating-colocation}
% \textit {It is difficult to gain a full view of group sketching in a distributed setting because online meetings are generally limited to one view per participant. In an attempt to create a real-time collaborative sketching experience, two team members tested a setup of two device cameras per person during a Zoom meeting.} 

% The setup included signing in to the meeting twice with two separate devices; one device was a PC camera aimed at the face of each participant and a second device was a phone camera that was directed on their paper and pen. Though it was awkward to find a suitable angle and stabilize the phone, facial expressions, gestures and gaze were captured along with a view of real time sketching. This method allowed the conversation to be held concurrently with a view of the sketching as it was unfolding within the discussion. This remote sketching activity was seamless in a virtual distributed design setup that simulated a co-located design environment. It supported conversational and visual communication, however, it was  cumbersome to recreate and was not attempted after this trial.
% There is considerable potential with developing better and easier ways to set up this type of distributed collaboration. For instance, this approach might mitigate lack of access to and experience with digital sketching tools such as Wacom tablet, and might make it more possible to use iPads.


% % \begin{figure}[tb]
% %   \centering
% %   \includegraphics[width=\columnwidth]{figures/sticky-notes-wall-miro2.png}
% %   \caption{This is an example of learning in progress. One designer reverted to a physical wall to gather their ideas on stickies, snap a photo and brought it into the Miro board (left). As a group, we wanted the re-positioning freedom of miro board stickies and remade made them to achieve this (right).}
% %   \label{fig:sticky-notes}
% % \end{figure}






% %\challengesection{C12. Testing Design Interactions}

% \challengesection{C9. Screen-Sharing to Collaborate in Software Applications}
% \textit {Different team members can use their software fluency and bring different skills to the table. With the goal of including everyone throughout the design process, we used screen-sharing via Zoom to collaborate in specialized environments such as designing in Adobe Illustrator or editing code.} 

% What made this method particularly useful was when there was skill cross-over in the team because meeting participants could be allowed to control the mouse during a screen-sharing session. For example A team member shared her design on the screen of an open Adobe Illustrator workspace during the Zoom meeting. Another team member controlled the mouse from a separate location on her shared Adobe Illustrator workspace. This process allowed for real time manipulation of visual components of our design by multiple members and skill sharing as well.

% Even in cases where collaborators were not manipulating the software remotely, we found sharing specialized environments to be useful as this tends to mimic casual co-located collaboration at work spaces. Designers will often gather around the work space of the person implementing a design to tweak position, padding, and other style details. We simulated this experience with screen-sharing, and being able to grant access to the mouse remotely meant that team members could point out these details with accuracy. 


% \newpage
% \challengesection{C10. Using Hand Gestures for Discussing Interaction}
% \textit {Animating designs using video or animation software is difficult for team members that lack such technical skills. Not everyone in the group knew how to digitally animate a design, which excluded some team members.}

% We discovered that the most accessible way for each team member to show their ideas was by talking camera-to-camera similar to a face-to-face co-located setting. The software knowledge gap was resolved by relying on hand gestures and moving static design artifacts with our hands while remaining visible in the camera. Everyone in the team with access to a web camera could speak to their ideas and show how they imagined the design would move with intuitive hand motions, facial expressions, sounds, pointing to, or moving their own sketches or cut outs while explaining their idea in front of the camera. This emphasized a fuller presence within a remote collaborative experience similar to that of a lab.

% We reflected on our choice of communicating about interactions and compared it to our previous visualization design experiences. Based on this, we think that we would have pointed to sketches instead of waving in the air if we had worked in a co-located mode of collaboration. We see the hand gestures as adding an extra barrier to communication about a topic that is already quite difficult. 
% % and assisted showing sketches over teleconferencing. We do note that showing sketches over teleconferencing does not work with virtual backgrounds. % capture diverse ideas. 




% % \challengesection{C12. Moving Static Components on a Miro board}
% \challengesection{C11. Lo-fi Prototyping for Visualization Interaction}
% \textit {It was challenging to find optimal tools to enable all of us to test interactions in a digital format given our variable programming expertise. We aimed to re-create the use of paper prototyping in a digital format that we would utilize in a co-located design session}

% To set up this session we utilized the collaborative digital whiteboard, Miro, as a "table top" space and exported assets from Illustrator to use as "paper" clippings. Teleconferencing with Zoom enabled gesturing and speaking into the camera, while simultaneously all team members could copy, resize and the arrange assets in Miro. Team members were able to collaboratively create UI mockups (Figure \ref{fig:prototyping-interactions-in-miro}) and animate them by clicking and dragging. We found this method to be quick and inclusive to all members, regardless of skill. Additionally, we found the ability to duplicate elements and groups of elements without disrupting the integrity of previous models actually provided a benefit over traditional paper prototyping.

% % While doing distributed visualization design posed challenging as we have described above, this mode of working also provided opportunities. Here, we outline experiences that either seemed as easy, or potentially easier than co-located design work. 


% % Being distributed forces you to be upfront about the process, and allow for later reflection because distributed work creates a repository

% % \opportunitysection{O1. Sharing design inspiration}

% % \opportunitysection{O2. Managing design artifacts}
% % The design meeting notes and artifacts were stored, categorized by date, and accessible in the software that we used. This cache of meeting notes and artifacts has proved to be simple and very useful when referring to previously posted resources or sketches during design meetings, especially for recalling what we did earlier and building upon our ideas.  For example, our sketches or national COVID-19 visualizations and meetings notes were Google Docs, Slack, or Miro that are invaluable to this paper because it allowed us to reflect on our record of detailed design activities enabling more insight to occur. 

% % \opportunitysection{O3. Keeping tabs on design provenance}
% % How the design came to be. Data about how we worked (Zoom data, Miro board history)



==> [BELIV 2020] Remote COVID-19 Design/sections/50-discussion.tex <==
%\newpage
\section{Discussion}
% Should the discussion be just for the VIS community?
As a team of information visualization designers we described and studied our experience using an auto-ethnographic approach in order to explore how we experienced visualization design methods in our project. Iterative reflection and thematic organization of our experiences presented us with overarching themes of challenges and strategies. During our pursuit to create a vibrant online collaboration in the early stages of visualization design, we were constantly reminded of situations that needed to be addressed, and that we felt were essential to maintain our co-located design process even though we were no longer able to meet in person. In doing so, we identified challenges and strategies that arose through our process, leading us to try new ways to conduct distributed synchronous collaboration. Our account may offer an example to the members of the visualization community who may identify with similar experiences that they too have had. This may serve to inform future visualization research and methodology in this domain.


We found that tools for designing, creating, and using visualizations such as Adobe Illustrator, RAW graphs~\cite{raw}, Tableau, Data Illustrator~\cite{liu2018data}, and Charticulator~\cite{ren2019charticulator} 
did not offer the support we were looking for in our synchronous collaboration. We more frequently relied on external web applications to collaborate both independently and together during our design sessions. We found the combined use of multiple applications such as teleconferencing (in our case, Zoom), virtual whiteboards (in our case, Miro), and collaborative word processors (in our case, Google Docs) provided considerable flexibility. However, constantly switching between applications became cumbersome at times, particularly when coordinating these between several team members during a teleconferencing session. Improved orchestration and integration between these applications, as well as more fine-tuned support for collaborative online sketching would be interesting directions to investigate and welcome improvements in such contexts.

In many design processes there are often activities that require the use of web tools or computing environments and for these we felt the shift to remote work did not hinder our performance of these activities. Research, data understanding, collaborative writing, finessing of high fidelity designs and prototypes are activities that often require the use of a computer. In a co-located scenario, we often have team members gather in a conference room with personal laptops that they must attach to an external display to properly share with the group, or gather at the shoulder of one team member while they informally demo something on their desktop. These types of in-person collaborative moments can be cumbersome. However, we found they happened more rapidly and comfortably over teleconferencing by utilizing built in tools such as screen sharing, or in combination with external collaborative software. 

We struggled more to adapt in the ideation and early iteration phases because our process relied on brainstorming, sketching, and rapid paper prototyping. We tried to mimic real-time collaborative sketching by setting up a dual screen conference, or by holding sketches up to the webcam.  To some extent, we were able to sustain spontaneity of brainstorming and idea sharing similar to those of co-located collaboration by continuing to use mostly physical sketching materials like pen and paper. The transfer of physical sketches to the virtual whiteboard was cumbersome and we see this as an area for potential improvement. However, once the sketches are on a digital whiteboard they continue to be accessible for all future discussions and are easily duplicated and iterated on much more easily than their physical counterparts. 
%We, as designers, needed to think critically about how to tell the story with the data as a way to communicate the complexity of the pandemic in the interest of ensuring that our visualisation would not be misinforming. Our critical discussions often referred to artifacts or relied on gestures and expressiveness that was difficult to convey via teleconference.
While we discussed access to equipment and distraction as being primarily a pandemic related challenge, we also see this as being potentially more widely problematic. Improvements we could make for our sketching sessions might involve high-quality webcams and sketching tablets for all team members. However, the cost and learning curve associated with adopting such technology is high considering that low-fi technology such as pen and paper work very efficiently and with more versatility. Likewise, having dedicated space and time to do one’s work is essential for focus, and offloading the responsibility to the individual to carve it out of their domestic space is understandably challenging for remote workers. 

Where we saw the largest challenge for remote work was communication and social dynamics. Working in a co-located environment facilitates serendipity, natural discussion, and a tangible sense of togetherness that allows for ideas to emerge spontaneously. We found some team members engaged in prolonged teleconferencing sessions to experience the sense of community and to concurrently share ideas as more of a ``hangout'' rather than a meeting. However, other team members who neither could nor chose to utilize video and did not engage in the ``hangouts'' slowly drifted away from the project likely because they felt excluded. In a co-located environment, it is quite clear that an individual is committed to working because they have physically arrived at work, and likewise one can pick up on how busy or idle a co-worker might be when they are co-located. Being disconnected to these physical cues, in conjunction with voluntary roles in our particular project, made assigning tasks or setting expectations challenging. We discovered that social dynamics that seamlessly sort themselves out in a co-located scenario require a lot more facilitation and management effort. We imagine that this may require an additional role or skill set added to a team, or better integration of a person's status (``available'', ``busy'', ``away'') into the collaborative environments. Messaging applications such as Slack provide status information, but in our experience, they lack nuance and integration with realistic highly synchronous workflows. There is no shortage of collaborative software that aims to increase productivity and facilitate focus sessions, but few that fulfill the sense of community and spontaneous collaboration that happens in co-located work environments. 

Finally, it is worth noting that the ability to reflect on our experience of synchronous distributed design is largely due to the fact that we were distributed. We were forced to put every piece of inspiration and every sketch into Miro. All of our notes and communications are documented on Slack and in Google docs. Having this detailed repository at every stage allowed us to reflect and gain insight into our process and learn from our experience. 

%%The ability to reflect on our experience of distributed design is largely due to the fact that we were distributed. We were forced to put every piece of inspiration and every sketch in Miro. All of our notes and communication are documented on Slack and in Google docs. Having this detailed repository at every stage allowed us to reflect and gain insight to our process and learn from our challenges.  
% \sarah{This part seems intended for conclusion:}
% While descriptions and discussions of visualization design has tended to assume co-located design teams, designers clearly need to carry out some work independently and in different locations. Prior work in other fields have shed light on this. However, there is important work to be done in considering these contexts for visualization design processes. We provide a first understanding and conceptualization of this area.
% \sarah {Can everything after this go?}
% he benefits of many of the applications extended beyond the synchronous collaboration sessions to individual work and to future collaborative sessions.
% Challenges of distributed collaboration
% Findings: solutions that worked to create a fluid remote collaboration
% Benefits of distributed synchronous collaboration
% Future applications and research
% In our work, we experienced benefits of using 
% Learning by reflecting on our collective experiences as cross-disciplinary designers. The online program Miro offered a common space to share our asynchronous sketches, reading materials, and other references during our synchronous online meetings. Google Docs was a repository of group documents such as design briefs and meeting notes. 
 
%  In order to support the process of ideation and data discovery, we wished to collaborate via a real-time sketching setup similar to co-located design environment such as a lab.  
 
 
%  Therefore, we pursued to create a  We searched for befitting tools and materials available to enable the team members to communicate ideas about interactions for the design and to share them, as we normally would, ‘in-person’. 
 
%  Design team
% Solutions that worked in other remote design and collaboration contexts
% - leveraging face-to-face interaction but using the camera
% - leveraging 'gestures'
% Similar challenges and solutions that we found in related work
% Being able to see real-time sketching from other team members
% Distinguishing different environments: co-located, distributed
% Team structure and work flow




% In our pursuit to create vibrant online infovis design it was essential that we are able to maintain our co-located design process as much as possible when were no longer able to meet in person. In doing so we discovered both challenges and benefits with virtual collaboration. Tools for designing, creating, and using visualizations such as Adobe Illustrator, RAW graphs, Tableau, Data Illustrator, Charticulator, offered little to no support for synchronous collaboration. We relied on external web applications to collaborate both independently and together during our design sessions. We found the combined use of multiple applications such as teleconferencing (for example, Zoom), virtual whiteboards (for example, Miro), and word processors (for example, Google Docs) provided great flexibility, but also became cumbersome at times to coordinate shifting between applications with multiple users during a single teleconferencing session. Improved orchestration and integration between these applications would be welcome. 

% In any design process there are activities that require the use of web tools or computing environments and for these we felt the shift to remote work did not hinder our performance of these activities. Research, data understanding, collaborative writing, finessing of high fidelity designs and prototypes are activities that often require the use of a computer. In a co-located scenario we often have team members gather in a conference room with personal laptops that they must attach to an external display to properly share with the group, or gather at the shoulder of one team member while they informally demo something on their desktop. These types of in person collaborative moments can be cumbersome, however, we found they happened more rapidly and comfortably over web conferencing by utilizing built in tools such as screen sharing, or in combination with external collaborative software. 

% We struggled to adapt more during the ideation and early iteration because our process relies on brainstorming, sketching, and rapid paper prototyping. We, as designers, needed to think critically about how to tell the story with the data as a way to communicate the complexity of the pandemic in the interest of ensuring that our visualisation would not be misinforming. Our critical discussions often refer to artifacts or rely on gestures and expressiveness that is difficult to convey via teleconference. We tried to mimic real-time collaborative sketching by setting up a dual screen conference, or by holding sketches up to the webcam.  We were able to sustain spontaneity of brain storming and idea sharing similar to those of co-located collaboration by continuing to use mostly physical sketching materials like pen and paper. The transfer of physical sketches to the virtual whiteboard was cumbersome and we see this as an area for potential improvement. However, once the sketches were on the digital whiteboard they continued to be accessible for all future discussions and are easily duplicated and iterated on much more easily than their physical counterparts. 

% While we discussed access to equipment and distraction as being primarily a pandemic related challenge in our case, we also see this potentially being more widely problematic as well. Improvements we could make for our sketching sessions might involve quality webcams and sketching tablets for all team members in the meeting. However, the cost and learning curve associated with adopting that technology is great considering that low-fi technology such as pen and paper works very efficiently and with more versatility. Likewise, having dedicated space and time to do ones work is essential for focus, and offloading the responsibility to the individual to carve it out of their domestic space is understandably challenging for remote workers. 

% Where we saw the largest challenge for remote work was communication and social dynamics. Working in a co-located environment facilitates serendipity, natural discussion and a tangible sense of togetherness that allows for ideas to spontaneously emerge. We found some team members would  engage in prolonged teleconferencing sessions to experience the sense of community and to spontaneously share ideas; more of a "hangout" than a meeting. However, other team members who either could not or chose not to utilize video, and did not engage in the "hangouts" slowly drifted away from the project, likely because they did not feel very included. In a co-located environment, it is quite clear that an individual is committed to working because they have physically arrived at work, and likewise one can pick up on how busy or idle a co-worker might be when they are co-located. Being disconnected to these physical cues, in conjunction with the our particular project being voluntary, made assigning tasks or setting expectations very challenging. We discovered that social dynamics that might sort themselves out in a co-located scenario require a lot more facilitation and management effort. We imagine that this may require an additional role or skill set added to a team, or better integration of a person's status into the collaborative environments. Messaging applications such as Slack utilize status ("available", "busy", "away") but this lacks nuance and integration with workflow. There is no shortage of collaborative software that aims to increase productivity and facilitate focus sessions, but few that fulfill the sense of community and spontaneous collaboration that happens in co-located work environments. 




% \sarah{This part seems intended for conclusion:}
% While descriptions and discussions of visualization design has tended to assume co-located design teams, designers clearly need to carry out some work independently and in different locations. Prior work in other fields have shed light on this. However, there is important work to be done in considering these contexts for visualization design processes. We provide a first understanding and conceptualization of this area.



% \sarah {Can everything after this go?}
% he benefits of many of the applications extended beyond the synchronous collaboration sessions to individual work and to future collaborative sessions.
% Challenges of distributed collaboration

% Findings: solutions that worked to create a fluid remote collaboration

% Benefits of distributed synchronous collaboration

% Future applications and research
% In our work, we experienced benefits of using 


% Learning by reflecting on our collective experiences as cross-disciplinary designers. The online program Miro offered a common space to share our asynchronous sketches, reading materials, and other references during our synchronous online meetings. Google Docs was a repository of group documents such as design briefs and meeting notes. 
 
%  In order to support the process of ideation and data discovery, we wished to collaborate via a real-time sketching setup similar to co-located design environment such as a lab.  
 
 
%  Therefore, we pursued to create a  We searched for befitting tools and materials available to enable the team members to communicate ideas about interactions for the design and to share them, as we normally would, ‘in-person’. 
 
%  Design team

% Solutions that worked in other remote design and collaboration contexts
% - leveraging face-to-face interaction but using the camera
% - leveraging 'gestures'

% Similar challenges and solutions that we found in related work

% Being able to see real-time sketching from other team members

% Distinguishing different environments: co-located, distributed

% Team structure and work flow









==> [BELIV 2020] Remote COVID-19 Design/sections/60-conclusion.tex <==
\section{Conclusion}
In this paper, we reflected on our experiences doing distributed visualization design in a remote synchronous design space during the pandemic. We based our reflections on our work on designing a COVID-19 visualization as part of a larger team effort on supporting city- and provincial-level decision-making. We discussed how the pandemic posed new challenges to remote collaboration amidst civic lockdown measures and imposed an increased dependency on spatially distributed teamwork across almost all sectors. As a response to the barriers of working from home being ``the new normal'', we used various synchronous remote design tools and methods with an aim to preserve the richness of co-located collaboration such as face-to-face physical presence with the ability to view real-time body gestures, facial expressions, and the making and sharing of physical artifacts. Based on these, we articulated issues in team composition and communication, both of which affected our visualization design process. We discussed the challenges of working in a distributed visualization design team, such as creating a sense of a shared work environment, which we liken to the idea of a design studio, and how to share data and potential ideas for visualization data. Finally, we offered potential solutions and benefits to working remotely. Our discovery of the challenges and strategies throughout the process provide useful insights about enabling a more fluid distributed collaboration.

While descriptions and discussions of visualization design tended to assume co-located design teams, designers clearly need to carry out some work independently and in different locations. Prior work in other fields have shed light on this. However, there is important work to be done in considering these contexts for visualization design processes. As a step towards developing a better understanding of distributed, synchronous visualization design, this paper provides an experiential understanding and conceptualization of this area.



==> [BELIV 2020] Remote COVID-19 Design/sections/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> [BELIV 2020] Remote COVID-19 Design/sections/from-template.tex <==
%% The ``\maketitle'' command must be the first command after the
%% ``\begin{document}'' command. It prepares and prints the title block.

%% the only exception to this rule is the \firstsection command
\firstsection{Introduction}

\maketitle

%% \section{Introduction} %for journal use above \firstsection{..} instead
This template is for papers of VGTC-sponsored conferences which are \emph{\textbf{not}} published in a special issue of TVCG.

\section{Using the Style Template}

\begin{itemize}
\item If you receive compilation errors along the lines of ``\texttt{Package ifpdf Error: Name clash, \textbackslash ifpdf is already defined}'' then please add a new line ``\texttt{\textbackslash let\textbackslash ifpdf\textbackslash relax}'' right after the ``\texttt{\textbackslash documentclass[journal]\{vgtc\}}'' call. Note that your error is due to packages you use that define ``\texttt{\textbackslash ifpdf}'' which is obsolete (the result is that \texttt{\textbackslash ifpdf} is defined twice); these packages should be changed to use ifpdf package instead.
\item The style uses the hyperref package, thus turns references into internal links. We thus recommend to make use of the ``\texttt{\textbackslash autoref\{reference\}}'' call (instead of ``\texttt{Figure\~{}\textbackslash ref\{reference\}}'' or similar) since ``\texttt{\textbackslash autoref\{reference\}}'' turns the entire reference into an internal link, not just the number. Examples: \autoref{fig:sample} and \autoref{tab:vis_papers}.
\item The style automatically looks for image files with the correct extension (eps for regular \LaTeX; pdf, png, and jpg for pdf\LaTeX), in a set of given subfolders (figures/, pictures/, images/). It is thus sufficient to use ``\texttt{\textbackslash includegraphics\{CypressView\}}'' (instead of ``\texttt{\textbackslash includegraphics\{pictures/CypressView.jpg\}}'').
\item For adding hyperlinks and DOIs to the list of references, you can use ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-hyperref-narrow\}}'' (instead of ``\texttt{\textbackslash bibliographystyle\{abbrv\}}''). It uses the doi and url fields in a bib\TeX\ entry and turns the entire reference into a link, giving priority to the doi. The doi can be entered with or without the ``\texttt{http://dx.doi.org/}'' url part. See the examples in the bib\TeX\ file and the bibliography at the end of this template.\\[1em]
\textbf{Note 1:} occasionally (for some \LaTeX\ distributions) this hyper-linked bib\TeX\ style may lead to \textbf{compilation errors} (``\texttt{pdfendlink ended up in different nesting level ...}'') if a reference entry is broken across two pages (due to a bug in hyperref). In this case make sure you have the latest version of the hyperref package (i.\,e., update your \LaTeX\ installation/packages) or, alternatively, revert back to ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-narrow\}}'' (at the expense of removing hyperlinks from the bibliography) and try ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-hyperref-narrow\}}'' again after some more editing.\\[1em]
\textbf{Note 2:} the ``\texttt{-narrow}'' versions of the bibliography style use the font ``PTSansNarrow-TLF'' for typesetting the DOIs in a compact way. This font needs to be available on your \LaTeX\ system. It is part of the \href{https://www.ctan.org/pkg/paratype}{``paratype'' package}, and many distributions (such as MikTeX) have it automatically installed. If you do not have this package yet and want to use a ``\texttt{-narrow}'' bibliography style then use your \LaTeX\ system's package installer to add it. If this is not possible you can also revert to the respective bibliography styles without the ``\texttt{-narrow}'' in the file name.\\[1em]
DVI-based processes to compile the template apparently cannot handle the different font so, by default, the template file uses the \texttt{abbrv-doi} bibliography style but the compiled PDF shows you the effect of the \texttt{abbrv-doi-hyperref-narrow} style.
\end{itemize}

\section{Bibliography Instructions}

\begin{itemize}
\item Sort all bibliographic entries alphabetically but the last name of the first author. This \LaTeX/bib\TeX\ template takes care of this sorting automatically.
\item Merge multiple references into one; e.\,g., use \cite{Max:1995:OMF,Kitware:2003} (not \cite{Kitware:2003}\cite{Max:1995:OMF}). Within each set of multiple references, the references should be sorted in ascending order. This \LaTeX/bib\TeX\ template takes care of both the merging and the sorting automatically.
\item Verify all data obtained from digital libraries, even ACM's DL and IEEE Xplore  etc.\ are sometimes wrong or incomplete.
\item Do not trust bibliographic data from other services such as Mendeley.com, Google Scholar, or similar; these are even more likely to be incorrect or incomplete.
\item Articles in journal---items to include:
  \begin{itemize}
  \item author names
	\item title
	\item journal name
	\item year
	\item volume
	\item number
	\item month of publication as variable name (i.\,e., \{jan\} for January, etc.; month ranges using \{jan \#\{/\}\# feb\} or \{jan \#\{-{}-\}\# feb\})
  \end{itemize}
\item use journal names in proper style: correct: ``IEEE Transactions on Visualization and Computer Graphics'', incorrect: ``Visualization and Computer Graphics, IEEE Transactions on''
\item Papers in proceedings---items to include:
  \begin{itemize}
  \item author names
	\item title
	\item abbreviated proceedings name: e.\,g., ``Proc.\textbackslash{} CONF\_ACRONYNM'' without the year; example: ``Proc.\textbackslash{} CHI'', ``Proc.\textbackslash{} 3DUI'', ``Proc.\textbackslash{} Eurographics'', ``Proc.\textbackslash{} EuroVis''
	\item year
	\item publisher
	\item town with country of publisher (the town can be abbreviated for well-known towns such as New York or Berlin)
  \end{itemize}
\item article/paper title convention: refrain from using curly brackets, except for acronyms/proper names/words following dashes/question marks etc.; example:
\begin{itemize}
	\item paper ``Marching Cubes: A High Resolution 3D Surface Construction Algorithm''
	\item should be entered as ``\{M\}arching \{C\}ubes: A High Resolution \{3D\} Surface Construction Algorithm'' or  ``\{M\}arching \{C\}ubes: A high resolution \{3D\} surface construction algorithm''
	\item will be typeset as ``Marching Cubes: A high resolution 3D surface construction algorithm''
\end{itemize}
\item for all entries
\begin{itemize}
	\item DOI can be entered in the DOI field as plain DOI number or as DOI url; alternative: a url in the URL field
	\item provide full page ranges AA-{}-BB
\end{itemize}
\item when citing references, do not use the reference as a sentence object; e.\,g., wrong: ``In \cite{Lorensen:1987:MCA} the authors describe \dots'', correct: ``Lorensen and Cline \cite{Lorensen:1987:MCA} describe \dots''
\end{itemize}

\section{Example Section}

Lorem\marginpar{\small You can use the margins for comments while editing the submission, but please remove the marginpar comments for submission.} ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam
voluptua~\cite{Kitware:2003,Max:1995:OMF}. At vero eos et accusam et
justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est.

\section{Exposition}

Duis autem vel eum iriure dolor in hendrerit in vulputate velit esse
molestie consequat, vel illum dolore eu feugiat nulla facilisis at
vero eros et accumsan et iusto odio dignissim qui blandit praesent
luptatum zzril delenit augue duis dolore te feugait nulla
facilisi. Lorem ipsum dolor sit amet, consectetuer adipiscing elit,
sed diam nonummy nibh euismod tincidunt ut laoreet dolore magna
aliquam erat volutpat~\cite{Kindlmann:1999:SAG}.

\begin{equation}
\sum_{j=1}^{z} j = \frac{z(z+1)}{2}
\end{equation}

Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet.

\subsection{Lorem ipsum}

Lorem ipsum dolor sit amet (see \autoref{tab:vis_papers}), consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. 

\begin{table}[tb]
  \caption{VIS/VisWeek accepted/presented papers: 1990--2016.}
  \label{tab:vis_papers}
  \scriptsize%
	\centering%
  \begin{tabu}{%
	r%
	*{7}{c}%
	*{2}{r}%
	}
  \toprule
   year & \rotatebox{90}{Vis/SciVis} &   \rotatebox{90}{SciVis conf} &   \rotatebox{90}{InfoVis} &   \rotatebox{90}{VAST} &   \rotatebox{90}{VAST conf} &   \rotatebox{90}{TVCG @ VIS} &   \rotatebox{90}{CG\&A @ VIS} &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{incl. TVCG/CG\&A}   &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{w/o TVCG/CG\&A}   \\
  \midrule
	2016 & 30 &   & 37 & 33 & 15 & 23 & 10 & 148 & 115 \\
  2015 & 33 & 9 & 38 & 33 & 14 & 17 & 15 & 159 & 127 \\
  2014 & 34 &   & 45 & 33 & 21 & 20 &   & 153 & 133 \\
  2013 & 31 &   & 38 & 32 &   & 20 &   & 121 & 101 \\
  2012 & 42 &   & 44 & 30 &   & 23 &   & 139 & 116 \\
  2011 & 49 &   & 44 & 26 &   & 20 &   & 139 & 119 \\
  2010 & 48 &   & 35 & 26 &   &   &   & 109 & 109 \\
  2009 & 54 &   & 37 & 26 &   &   &   & 117 & 117 \\
  2008 & 50 &   & 28 & 21 &   &   &   & 99 & 99 \\
  2007 & 56 &   & 27 & 24 &   &   &   & 107 & 107 \\
  2006 & 63 &   & 24 & 26 &   &   &   & 113 & 113 \\
  2005 & 88 &   & 31 &   &   &   &   & 119 & 119 \\
  2004 & 70 &   & 27 &   &   &   &   & 97 & 97 \\
  2003 & 74 &   & 29 &   &   &   &   & 103 & 103 \\
  2002 & 78 &   & 23 &   &   &   &   & 101 & 101 \\
  2001 & 74 &   & 22 &   &   &   &   & 96 & 96 \\
  2000 & 73 &   & 20 &   &   &   &   & 93 & 93 \\
  1999 & 69 &   & 19 &   &   &   &   & 88 & 88 \\
  1998 & 72 &   & 18 &   &   &   &   & 90 & 90 \\
  1997 & 72 &   & 16 &   &   &   &   & 88 & 88 \\
  1996 & 65 &   & 12 &   &   &   &   & 77 & 77 \\
  1995 & 56 &   & 18 &   &   &   &   & 74 & 74 \\
  1994 & 53 &   &   &   &   &   &   & 53 & 53 \\
  1993 & 55 &   &   &   &   &   &   & 55 & 55 \\
  1992 & 53 &   &   &   &   &   &   & 53 & 53 \\
  1991 & 50 &   &   &   &   &   &   & 50 & 50 \\
  1990 & 53 &   &   &   &   &   &   & 53 & 53 \\
  \midrule
  \textbf{sum} & \textbf{1545} & \textbf{9} & \textbf{632} & \textbf{310} & \textbf{50} & \textbf{123} & \textbf{25} & \textbf{2694} & \textbf{2546} \\
  \bottomrule
  \end{tabu}%
\end{table}

\subsection{Mezcal Head}

Lorem ipsum dolor sit amet (see \autoref{fig:sample}), consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. 

\subsubsection{Duis Autem}

Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est. Lorem
ipsum dolor sit amet.

\begin{figure}[tb]
 \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
 \includegraphics[width=\columnwidth]{paper-count-w-2015-new}
 \caption{A visualization of the 1990--2015 data from \autoref{tab:vis_papers}. The image is from \cite{Isenberg:2017:VMC} and is in the public domain.}
 \label{fig:sample}
\end{figure}

See Figure \ref{fig:sample}.

\subsubsection{Ejector Seat Reservation}

Duis autem~\cite{Lorensen:1987:MCA}\footnote{The algorithm behind
Marching Cubes \cite{Lorensen:1987:MCA} had already been
described by Wyvill et al. \cite{Wyvill:1986:DSS} a year
earlier.} vel eum iriure dolor in hendrerit
in vulputate velit esse molestie consequat,\footnote{Footnotes
appear at the bottom of the column.} vel illum dolore eu
feugiat nulla facilisis at vero eros et accumsan et iusto odio
dignissim qui blandit praesent luptatum zzril delenit augue duis
dolore te feugait nulla facilisi. Lorem ipsum dolor sit amet,
consectetuer adipiscing elit, sed diam nonummy nibh euismod tincidunt
ut laoreet dolore magna aliquam erat volutpat.


\paragraph{Confirmed Ejector Seat Reservation}

Ut wisi enim ad minim veniam, quis nostrud exerci tation ullamcorper
suscipit lobortis nisl ut aliquip ex ea commodo
consequat~\cite{Nielson:1991:TAD}. Duis autem vel eum iriure dolor in
hendrerit in vulputate velit esse molestie consequat, vel illum dolore
eu feugiat nulla facilisis at vero eros et accumsan et iusto odio
dignissim qui blandit praesent luptatum zzril delenit augue duis
dolore te feugait nulla facilisi.

\paragraph{Rejected Ejector Seat Reservation}

Ut wisi enim ad minim veniam, quis nostrud exerci tation ullamcorper
suscipit lobortis nisl ut aliquip ex ea commodo consequat. Duis autem
vel eum iriure dolor in hendrerit in vulputate velit esse molestie


\section{Conclusion}

Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum.



==> [BELIV 2020] Remote COVID-19 Design/sections/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> [BELIV 2020] Remote COVID-19 Design/todo.tex <==
Table 1 could  be improved, add citations from vis to table, potentially make more visually appealing in Illustrator
Table 2 make more visually appealing in Illustrator

Challenges: 
Consider condensing/removing challenges
Make Challenges and opportunities fit together more consistently

Create figure that shows various sketching media (pen+paper, iPad app(s), Illustrator, prototypes)

Related work could be improved/extended 

Acknowledgments: Add funding sources, Neil, Jackie, Center people

Figure showing a version of Figure 1 (teaser) but with COVID Task Force meetings

Rename "design" and "larger team"

Take a critical look at title+abstract

Once challenges and opportunities are done, make sure that title+abstract+intro+discussion+conclusion matches

Software prototyping section could be improved+expanded. Think about how this relates to the challenges

Sprinkle citations throughout









==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> sections/from-template.tex <==
%% The ``\maketitle'' command must be the first command after the
%% ``\begin{document}'' command. It prepares and prints the title block.

%% the only exception to this rule is the \firstsection command
\firstsection{Introduction}

\maketitle

%% \section{Introduction} %for journal use above \firstsection{..} instead
This template is for papers of VGTC-sponsored conferences which are \emph{\textbf{not}} published in a special issue of TVCG.

\section{Using the Style Template}

\begin{itemize}
\item If you receive compilation errors along the lines of ``\texttt{Package ifpdf Error: Name clash, \textbackslash ifpdf is already defined}'' then please add a new line ``\texttt{\textbackslash let\textbackslash ifpdf\textbackslash relax}'' right after the ``\texttt{\textbackslash documentclass[journal]\{vgtc\}}'' call. Note that your error is due to packages you use that define ``\texttt{\textbackslash ifpdf}'' which is obsolete (the result is that \texttt{\textbackslash ifpdf} is defined twice); these packages should be changed to use ifpdf package instead.
\item The style uses the hyperref package, thus turns references into internal links. We thus recommend to make use of the ``\texttt{\textbackslash autoref\{reference\}}'' call (instead of ``\texttt{Figure\~{}\textbackslash ref\{reference\}}'' or similar) since ``\texttt{\textbackslash autoref\{reference\}}'' turns the entire reference into an internal link, not just the number. Examples: \autoref{fig:sample} and \autoref{tab:vis_papers}.
\item The style automatically looks for image files with the correct extension (eps for regular \LaTeX; pdf, png, and jpg for pdf\LaTeX), in a set of given subfolders (figures/, pictures/, images/). It is thus sufficient to use ``\texttt{\textbackslash includegraphics\{CypressView\}}'' (instead of ``\texttt{\textbackslash includegraphics\{pictures/CypressView.jpg\}}'').
\item For adding hyperlinks and DOIs to the list of references, you can use ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-hyperref-narrow\}}'' (instead of ``\texttt{\textbackslash bibliographystyle\{abbrv\}}''). It uses the doi and url fields in a bib\TeX\ entry and turns the entire reference into a link, giving priority to the doi. The doi can be entered with or without the ``\texttt{http://dx.doi.org/}'' url part. See the examples in the bib\TeX\ file and the bibliography at the end of this template.\\[1em]
\textbf{Note 1:} occasionally (for some \LaTeX\ distributions) this hyper-linked bib\TeX\ style may lead to \textbf{compilation errors} (``\texttt{pdfendlink ended up in different nesting level ...}'') if a reference entry is broken across two pages (due to a bug in hyperref). In this case make sure you have the latest version of the hyperref package (i.\,e., update your \LaTeX\ installation/packages) or, alternatively, revert back to ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-narrow\}}'' (at the expense of removing hyperlinks from the bibliography) and try ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-hyperref-narrow\}}'' again after some more editing.\\[1em]
\textbf{Note 2:} the ``\texttt{-narrow}'' versions of the bibliography style use the font ``PTSansNarrow-TLF'' for typesetting the DOIs in a compact way. This font needs to be available on your \LaTeX\ system. It is part of the \href{https://www.ctan.org/pkg/paratype}{``paratype'' package}, and many distributions (such as MikTeX) have it automatically installed. If you do not have this package yet and want to use a ``\texttt{-narrow}'' bibliography style then use your \LaTeX\ system's package installer to add it. If this is not possible you can also revert to the respective bibliography styles without the ``\texttt{-narrow}'' in the file name.\\[1em]
DVI-based processes to compile the template apparently cannot handle the different font so, by default, the template file uses the \texttt{abbrv-doi} bibliography style but the compiled PDF shows you the effect of the \texttt{abbrv-doi-hyperref-narrow} style.
\end{itemize}

\section{Bibliography Instructions}

\begin{itemize}
\item Sort all bibliographic entries alphabetically but the last name of the first author. This \LaTeX/bib\TeX\ template takes care of this sorting automatically.
\item Merge multiple references into one; e.\,g., use \cite{Max:1995:OMF,Kitware:2003} (not \cite{Kitware:2003}\cite{Max:1995:OMF}). Within each set of multiple references, the references should be sorted in ascending order. This \LaTeX/bib\TeX\ template takes care of both the merging and the sorting automatically.
\item Verify all data obtained from digital libraries, even ACM's DL and IEEE Xplore  etc.\ are sometimes wrong or incomplete.
\item Do not trust bibliographic data from other services such as Mendeley.com, Google Scholar, or similar; these are even more likely to be incorrect or incomplete.
\item Articles in journal---items to include:
  \begin{itemize}
  \item author names
	\item title
	\item journal name
	\item year
	\item volume
	\item number
	\item month of publication as variable name (i.\,e., \{jan\} for January, etc.; month ranges using \{jan \#\{/\}\# feb\} or \{jan \#\{-{}-\}\# feb\})
  \end{itemize}
\item use journal names in proper style: correct: ``IEEE Transactions on Visualization and Computer Graphics'', incorrect: ``Visualization and Computer Graphics, IEEE Transactions on''
\item Papers in proceedings---items to include:
  \begin{itemize}
  \item author names
	\item title
	\item abbreviated proceedings name: e.\,g., ``Proc.\textbackslash{} CONF\_ACRONYNM'' without the year; example: ``Proc.\textbackslash{} CHI'', ``Proc.\textbackslash{} 3DUI'', ``Proc.\textbackslash{} Eurographics'', ``Proc.\textbackslash{} EuroVis''
	\item year
	\item publisher
	\item town with country of publisher (the town can be abbreviated for well-known towns such as New York or Berlin)
  \end{itemize}
\item article/paper title convention: refrain from using curly brackets, except for acronyms/proper names/words following dashes/question marks etc.; example:
\begin{itemize}
	\item paper ``Marching Cubes: A High Resolution 3D Surface Construction Algorithm''
	\item should be entered as ``\{M\}arching \{C\}ubes: A High Resolution \{3D\} Surface Construction Algorithm'' or  ``\{M\}arching \{C\}ubes: A high resolution \{3D\} surface construction algorithm''
	\item will be typeset as ``Marching Cubes: A high resolution 3D surface construction algorithm''
\end{itemize}
\item for all entries
\begin{itemize}
	\item DOI can be entered in the DOI field as plain DOI number or as DOI url; alternative: a url in the URL field
	\item provide full page ranges AA-{}-BB
\end{itemize}
\item when citing references, do not use the reference as a sentence object; e.\,g., wrong: ``In \cite{Lorensen:1987:MCA} the authors describe \dots'', correct: ``Lorensen and Cline \cite{Lorensen:1987:MCA} describe \dots''
\end{itemize}

\section{Example Section}

Lorem\marginpar{\small You can use the margins for comments while editing the submission, but please remove the marginpar comments for submission.} ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam
voluptua~\cite{Kitware:2003,Max:1995:OMF}. At vero eos et accusam et
justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est.

\section{Exposition}

Duis autem vel eum iriure dolor in hendrerit in vulputate velit esse
molestie consequat, vel illum dolore eu feugiat nulla facilisis at
vero eros et accumsan et iusto odio dignissim qui blandit praesent
luptatum zzril delenit augue duis dolore te feugait nulla
facilisi. Lorem ipsum dolor sit amet, consectetuer adipiscing elit,
sed diam nonummy nibh euismod tincidunt ut laoreet dolore magna
aliquam erat volutpat~\cite{Kindlmann:1999:SAG}.

\begin{equation}
\sum_{j=1}^{z} j = \frac{z(z+1)}{2}
\end{equation}

Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet.

\subsection{Lorem ipsum}

Lorem ipsum dolor sit amet (see \autoref{tab:vis_papers}), consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. 

\begin{table}[tb]
  \caption{VIS/VisWeek accepted/presented papers: 1990--2016.}
  \label{tab:vis_papers}
  \scriptsize%
	\centering%
  \begin{tabu}{%
	r%
	*{7}{c}%
	*{2}{r}%
	}
  \toprule
   year & \rotatebox{90}{Vis/SciVis} &   \rotatebox{90}{SciVis conf} &   \rotatebox{90}{InfoVis} &   \rotatebox{90}{VAST} &   \rotatebox{90}{VAST conf} &   \rotatebox{90}{TVCG @ VIS} &   \rotatebox{90}{CG\&A @ VIS} &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{incl. TVCG/CG\&A}   &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{w/o TVCG/CG\&A}   \\
  \midrule
	2016 & 30 &   & 37 & 33 & 15 & 23 & 10 & 148 & 115 \\
  2015 & 33 & 9 & 38 & 33 & 14 & 17 & 15 & 159 & 127 \\
  2014 & 34 &   & 45 & 33 & 21 & 20 &   & 153 & 133 \\
  2013 & 31 &   & 38 & 32 &   & 20 &   & 121 & 101 \\
  2012 & 42 &   & 44 & 30 &   & 23 &   & 139 & 116 \\
  2011 & 49 &   & 44 & 26 &   & 20 &   & 139 & 119 \\
  2010 & 48 &   & 35 & 26 &   &   &   & 109 & 109 \\
  2009 & 54 &   & 37 & 26 &   &   &   & 117 & 117 \\
  2008 & 50 &   & 28 & 21 &   &   &   & 99 & 99 \\
  2007 & 56 &   & 27 & 24 &   &   &   & 107 & 107 \\
  2006 & 63 &   & 24 & 26 &   &   &   & 113 & 113 \\
  2005 & 88 &   & 31 &   &   &   &   & 119 & 119 \\
  2004 & 70 &   & 27 &   &   &   &   & 97 & 97 \\
  2003 & 74 &   & 29 &   &   &   &   & 103 & 103 \\
  2002 & 78 &   & 23 &   &   &   &   & 101 & 101 \\
  2001 & 74 &   & 22 &   &   &   &   & 96 & 96 \\
  2000 & 73 &   & 20 &   &   &   &   & 93 & 93 \\
  1999 & 69 &   & 19 &   &   &   &   & 88 & 88 \\
  1998 & 72 &   & 18 &   &   &   &   & 90 & 90 \\
  1997 & 72 &   & 16 &   &   &   &   & 88 & 88 \\
  1996 & 65 &   & 12 &   &   &   &   & 77 & 77 \\
  1995 & 56 &   & 18 &   &   &   &   & 74 & 74 \\
  1994 & 53 &   &   &   &   &   &   & 53 & 53 \\
  1993 & 55 &   &   &   &   &   &   & 55 & 55 \\
  1992 & 53 &   &   &   &   &   &   & 53 & 53 \\
  1991 & 50 &   &   &   &   &   &   & 50 & 50 \\
  1990 & 53 &   &   &   &   &   &   & 53 & 53 \\
  \midrule
  \textbf{sum} & \textbf{1545} & \textbf{9} & \textbf{632} & \textbf{310} & \textbf{50} & \textbf{123} & \textbf{25} & \textbf{2694} & \textbf{2546} \\
  \bottomrule
  \end{tabu}%
\end{table}

\subsection{Mezcal Head}

Lorem ipsum dolor sit amet (see \autoref{fig:sample}), consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. 

\subsubsection{Duis Autem}

Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est. Lorem
ipsum dolor sit amet.

\begin{figure}[tb]
 \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
 \includegraphics[width=\columnwidth]{paper-count-w-2015-new}
 \caption{A visualization of the 1990--2015 data from \autoref{tab:vis_papers}. The image is from \cite{Isenberg:2017:VMC} and is in the public domain.}
 \label{fig:sample}
\end{figure}

See Figure \ref{fig:sample}.

\subsubsection{Ejector Seat Reservation}

Duis autem~\cite{Lorensen:1987:MCA}\footnote{The algorithm behind
Marching Cubes \cite{Lorensen:1987:MCA} had already been
described by Wyvill et al. \cite{Wyvill:1986:DSS} a year
earlier.} vel eum iriure dolor in hendrerit
in vulputate velit esse molestie consequat,\footnote{Footnotes
appear at the bottom of the column.} vel illum dolore eu
feugiat nulla facilisis at vero eros et accumsan et iusto odio
dignissim qui blandit praesent luptatum zzril delenit augue duis
dolore te feugait nulla facilisi. Lorem ipsum dolor sit amet,
consectetuer adipiscing elit, sed diam nonummy nibh euismod tincidunt
ut laoreet dolore magna aliquam erat volutpat.


\paragraph{Confirmed Ejector Seat Reservation}

Ut wisi enim ad minim veniam, quis nostrud exerci tation ullamcorper
suscipit lobortis nisl ut aliquip ex ea commodo
consequat~\cite{Nielson:1991:TAD}. Duis autem vel eum iriure dolor in
hendrerit in vulputate velit esse molestie consequat, vel illum dolore
eu feugiat nulla facilisis at vero eros et accumsan et iusto odio
dignissim qui blandit praesent luptatum zzril delenit augue duis
dolore te feugait nulla facilisi.

\paragraph{Rejected Ejector Seat Reservation}

Ut wisi enim ad minim veniam, quis nostrud exerci tation ullamcorper
suscipit lobortis nisl ut aliquip ex ea commodo consequat. Duis autem
vel eum iriure dolor in hendrerit in vulputate velit esse molestie


\section{Conclusion}

Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
invidunt ut labore et dolore magna aliquyam erat, sed diam
voluptua. At vero eos et accusam et justo duo dolores et ea
rebum.



==> sections/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> todo.tex <==
Table 1 could  be improved, add citations from vis to table, potentially make more visually appealing in Illustrator
Table 2 make more visually appealing in Illustrator

Challenges: 
Consider condensing/removing challenges
Make Challenges and opportunities fit together more consistently

Create figure that shows various sketching media (pen+paper, iPad app(s), Illustrator, prototypes)

Related work could be improved/extended 

Acknowledgments: Add funding sources, Neil, Jackie, Center people

Figure showing a version of Figure 1 (teaser) but with COVID Task Force meetings

Rename "design" and "larger team"

Take a critical look at title+abstract

Once challenges and opportunities are done, make sure that title+abstract+intro+discussion+conclusion matches

Software prototyping section could be improved+expanded. Think about how this relates to the challenges

Sprinkle citations throughout








